LSVD: Loss-Aware Low-Rank Approximation for Efficient Low-Precision Vision-Language Models

Vision-language models (VLMs) deliver strong multimodal reasoning capabilities, but their large computational cost and high parameter counts make deployment challenging on resource-constrained devices. Low-rank decomposition has emerged as a promising compression technique, yet existing methods often optimize local matrix reconstruction error, rely on uniform or heuristic rank allocation, and focus mainly on attention projections while leaving feed-forward networks underexplored. In this paper, we propose~\textit{LASER} (\textbf{L}oss-\textbf{A}ware \textbf{S}ingular-value d\textbf{E}composition and \textbf{R}ank allocation), a low-rank compression framework for efficient low-precision VLM inference. LASER derives a curvature-weighted SVD objective from a second-order approximation of the model loss and uses Kronecker-factored Fisher information to guide decomposition toward downstream performance rather than reconstruction alone. We further introduce a loss-aware cross-layer rank allocation strategy based on calibration gradients, enabling more effective parameter budgeting across layers. Finally, we extend low-rank compression to FFN layers through a hybrid scheme that combines SVD with quantization. The evaluation results show that LASER achieves more than $2.3\times$ decoding speedup over previous work while preserving strong accuracy under low-precision inference.

==> draft.tex <==
\subsection{Loss-Aware Singular Value Decomposition}
\label{sec:loss-aware-svd}
Building on Section~\ref{sec:loss-aware-lra}, consider a linear layer with weight $W\in\mathbb{R}^{m\times n}$ and its rank-$r$ approximation $\widehat{W}$. The loss variation caused by the compression perturbation $\Delta W=\widehat{W}-W$ can be approximated using the Kronecker-factored curvature surrogate:
{\small
\begin{equation}
\Delta \mathcal{L}
\approx
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
(G\otimes X)
\mathrm{vec}(\Delta W)
\end{equation}}
where $X$ and $G$ are the activation and gradient covariance factors. Let $X=S_x^{\top}S_x$ and $G=S_gS_g^{\top}$
% {\small
% \begin{equation}
% X=S_xS_x^{\top},
% \qquad
% G=S_g^{\top}S_g
% \end{equation}}
be positive semi-definite factorizations of the curvature factors. In practice, $S_x$ and $S_g$ can be obtained by Cholesky decomposition~\cite{higham1990analysis} or by eigenvalue decomposition~\cite{abdi2007eigen} from $X$ and $G$. Using the standard identities of Kronecker product: $(A\otimes B)(C\otimes D)=(AC)\otimes(BD)$ and $\mathrm{vec}(ABC)=(C^{\top}\otimes A)\mathrm{vec}(B)$, we obtain:
{\small
\begin{flalign}
\Delta \mathcal{L}
&\approx
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
(G\otimes X)
\mathrm{vec}(\Delta W) \nonumber\\
&=
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
(S_gS_g^{\top}\otimes S_x^{\top}S_x)
\mathrm{vec}(\Delta W) \nonumber=
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
(S_g\otimes S_x^{\top})
(S_g^{\top}\otimes S_x)
\mathrm{vec}(\Delta W) \nonumber\\
&=
\frac{1}{2}
\left[
(S_g^{\top}\otimes S_x)
\mathrm{vec}(\Delta W)
\right]^{\top}
\left[
(S_g^{\top}\otimes S_x)
\mathrm{vec}(\Delta W)
\right] \nonumber=
\frac{1}{2}
\mathrm{vec}(S_x\Delta W S_g)^{\top}
\mathrm{vec}(S_x\Delta W S_g) \nonumber\\
&=
\frac{1}{2}
\left\|
S_x\Delta W S_g
\right\|_F^2
&&
\end{flalign}}



Thus, minimizing the second-order loss surrogate leads to a
curvature-weighted low-rank approximation problem:
{\small
\begin{equation}
\widehat{W}^{\star}
=
\arg\min_{\mathrm{rank}(\widehat{W})\le r}
\left\|
S_x(W-\widehat{W})S_g
\right\|_F^2
\end{equation}}

This weighted objective can be reduced to a standard Frobenius-norm low-rank approximation in a transformed weight space. Assuming the curvature factors $S_x$ and $S_g$ are nonsingular, we define the curvature-weighted matrix as $\widetilde{W}=S_x W S_g$. For any feasible rank-r approximation $\widehat{W}_r$, its transformed counterpart is $\widetilde{W}_r=S_x \widehat{W}_r S_g$. Because multiplication by nonsingular matrices preserves rank, this transformation establishes a one-to-one correspondence between rank-r solutions in the original parameter space and those in the curvature-weighted space. Therefore, the original weighted approximation problem is equivalent to the following standard low-rank approximation problem:

{\small
\begin{equation}
\min_{\mathrm{rank}(\widetilde{W}_r)\le r}
\left\|
\widetilde{W}-\widetilde{W}_r
\right\|_F^2
\end{equation}}

By the Eckart--Young--Mirsky theorem~\cite{eckart1936approximation,mirsky1960symmetric},
the optimal solution is obtained by applying truncated SVD to the
curvature-weighted weight matrix $\widetilde{W}=S_x W S_g$, rather than to the
original weight matrix $W$. Specifically, applying SVD to $\widetilde{W}$
yields:
{\small
\begin{equation}
\operatorname{SVD}(\widetilde{W})=U\Sigma V^{\top},
\qquad
\Sigma=\mathrm{diag}(\sigma_1,\ldots,\sigma_q),
\qquad
\sigma_1\ge \cdots \ge \sigma_q \ge 0
\end{equation}}
where $\Sigma$ is the diagonal matrix of singular values sorted in descending
order, and $q=\min\{m,n\}$ is the maximum possible rank. The optimal rank-$r$
approximation in the curvature-weighted space is obtained by retaining the top
$r$ singular components:
$\widetilde{W}_r^{\star}=U_r\Sigma_rV_r^{\top}$, where
$U_r$, $\Sigma_r$, and $V_r$ denote the corresponding truncated factors.
While $\widetilde{W}_r^{\star}$ solves the transformed approximation problem,
the actual compressed weight used in the model must be expressed in the
original parameter space. Therefore, we map it back through the inverse
curvature transformations:
{\small
\begin{equation}
\widehat{W}_r^{\star}
=
S_x^{-1}U_r\Sigma_rV_r^{\top}S_g^{-1}
=
A_rB_r,
\qquad
A_r=S_x^{-1}U_r\Sigma_r^{1/2},
\quad
B_r=\Sigma_r^{1/2}V_r^{\top}S_g^{-1}
\end{equation}}

In deployment, we execute the compressed layer in factorized form rather than
materializing $\widehat{W}_r^{\star}\in\mathbb{R}^{m\times n}$: the dense
operation $xW$ is replaced by $xA_rB_r$, where
$A_r\in\mathbb{R}^{m\times r}$ and $B_r\in\mathbb{R}^{r\times n}$. This reduces
the parameter count and dominant MAC cost from
$\alpha_{\mathrm{dense}}=mn$ to $\alpha_{\mathrm{svd}}=mr+rn$. We denote the
corresponding ratio by
$\rho_1=\alpha_{\mathrm{svd}}/\alpha_{\mathrm{dense}}=r(m+n)/(mn)$.
Thus, the factorized layer is more efficient than the dense layer when
$\rho_1<1$, equivalently $r<mn/(m+n)$. (\textcolor{red}{needs some clarification})
Moreover, the truncated singular values provide a closed-form expression for both the Frobenius residual in the curvature-weighted space and the corresponding second-order loss estimate. Since $\widetilde{W}=S_xWS_g$ and
$\widetilde{W}_r^{\star}=S_x\widehat{W}_r^{\star}S_g$, the perturbation
$\Delta W_r^{\star}=\widehat{W}_r^{\star}-W$ satisfies:
{\small
\begin{equation}
\left\|
\widetilde{W}-\widetilde{W}_r^{\star}
\right\|_F^2
=
\sum_{i=r+1}^{q}\sigma_i^2,
\qquad
\Delta \mathcal{L}_r
\approx
\frac{1}{2}
\left\|
S_x\Delta W_r^{\star}S_g
\right\|_F^2
=
\frac{1}{2}
\left\|
\widetilde{W}_r^{\star}-\widetilde{W}
\right\|_F^2
=
\frac{1}{2}
\sum_{i=r+1}^{q}\sigma_i^2
\label{eq:trunc-loss}
\end{equation}}

\subsection{Loss-Aware Cross-Layer Rank Allocation}
\label{sec:rank-alloc}
Although Eq.~\ref{eq:trunc-loss} provides a closed-form truncation-loss estimate
for each curvature-weighted matrix, these estimates are not necessarily
comparable across layers. Specifically, discarding the $i$-th singular component
of layer $\ell$ induces a K-FAC-based loss estimate of
$\frac{1}{2}\sigma_{\ell,i}^2$. A natural global rank-allocation rule would
therefore pool all singular components across layers and discard those with the
smallest $\sigma_{\ell,i}^2$. This rule, however, is well calibrated only if the
K-FAC surrogates of different layers place their singular values on a shared
loss scale.
The key challenge is that K-FAC provides a \textbf{layer-wise local curvature approximation}, rather than a globally calibrated curvature metric across layers. Denote the empirical Fisher block of layer $\ell$ by $F_\ell$, and its K-FAC approximation by $K_\ell=G_\ell\otimes X_\ell$, where $X_\ell$ and $G_\ell$ are the activation and output-gradient covariance factors. For the perturbation $\Delta W_{\ell,i}$ induced by discarding the $i$-th singular component, define $v_{\ell,i}=\operatorname{vec}(\Delta W_{\ell,i})$, where $\operatorname{vec}(\cdot)$ stacks the columns of a matrix into a vector. Then, by writing $F_\ell=K_\ell+(F_\ell-K_\ell)$, the empirical-Fisher second-order loss contribution decomposes into a K-FAC term and a residual term:
{\small
\begin{equation}
\Delta \mathcal{L}^{F}_{\ell,i}
\approx
\frac{1}{2}v_{\ell,i}^{\top}K_\ell v_{\ell,i}
+
\frac{1}{2}v_{\ell,i}^{\top}(F_\ell-K_\ell)v_{\ell,i}
\triangleq
T^{\mathrm{KFAC}}_{\ell,i}+T^{\mathrm{res}}_{\ell,i}
\label{eq:kfac-error-decomp}
\end{equation}}

The first term, $T^{\mathrm{KFAC}}_{\ell,i}$, is exactly the loss surrogate optimized by the K-FAC-based curvature-weighted SVD in Sec.~\ref{sec:loss-aware-svd}. For the $i$-th discarded singular component, this term reduces to
$T^{\mathrm{KFAC}}_{\ell,i}=\frac{1}{2}\sigma_{\ell,i}^{2}$. The second term, $T^{\mathrm{res}}_{\ell,i}$, is the approximation residual caused by replacing the empirical Fisher $F_\ell$ with its Kronecker-factored surrogate $K_\ell$. Therefore, directly comparing $\sigma_{\ell,i}^{2}$ across layers implicitly assumes that these residuals are either negligible or similarly scaled across layers.

Since $T^{\mathrm{res}}_{\ell,i}$ depends on the perturbation vector
$v_{\ell,i}$, exactly evaluating it for every discarded singular component would
require the full empirical Fisher. To avoid this cost, we use a direction-averaged
curvature-scale comparison between $F_\ell$ and $K_\ell$. Consider a generic
perturbation $v=a u$, where $u\in\mathbb{R}^{d_\ell}$ is a random isotropic unit
direction satisfying $\mathbb{E}[uu^\top]=I/d_\ell$, and $a$ is a nonzero
perturbation magnitude. For any square matrix $C$,
$\mathbb{E}[(au)^\top C(au)]
=
a^2\mathrm{Tr}(C)/d_\ell $. Thus, the trace characterizes
the direction-averaged quadratic curvature scale. Applying this identity to $F_\ell-K_\ell$
and $K_\ell$, the expected residual normalized by the expected K-FAC term becomes:
{\small
\begin{equation}
\frac{
\mathbb{E}\!\left[
\frac{1}{2}(a u)^\top(F_\ell-K_\ell)(a u)
\right]
}{
\mathbb{E}\!\left[
\frac{1}{2}(a u)^\top K_\ell (a u)
\right]
}
=
\frac{
\frac{a^2}{2}\mathrm{Tr}(F_\ell-K_\ell)/d_\ell
}{
\frac{a^2}{2}\mathrm{Tr}(K_\ell)/d_\ell
} 
=
\frac{\mathrm{Tr}(F_\ell)-\mathrm{Tr}(K_\ell)}
{\mathrm{Tr}(K_\ell)}
=
\eta_\ell-1 ,
\label{eq:avg-relative-residual}
\end{equation}}
{\small
\begin{equation}
\eta_\ell
\triangleq
\frac{\mathrm{Tr}(F_\ell)}{\mathrm{Tr}(K_\ell)}
=
\frac{\mathrm{Tr}(F_\ell)}
{\mathrm{Tr}(G_\ell\otimes X_\ell)}
=
\frac{\mathrm{Tr}(F_\ell)}
{\mathrm{Tr}(G_\ell)\mathrm{Tr}(X_\ell)}
\label{eq:eta-definition}
\end{equation}}

Thus, the ratio $\eta_\ell$ should be interpreted as an average scale check for the
K-FAC surrogate. Specifically, $\eta_\ell>1$ means that $K_\ell$ underestimates
the direction-averaged empirical-Fisher quadratic form of layer $\ell$, while
$\eta_\ell<1$ means that it overestimates it. Since the ratio is averaged over
generic isotropic perturbations, it is not a per-component correction for
$T^{\mathrm{res}}_{\ell,i}$. Instead, it measures whether the K-FAC truncation
loss assigns the correct average loss scale to a layer. Therefore,
$\sigma_{\ell,i}^{2}$ can still be meaningful for comparing singular components
within the same layer, but may be miscalibrated for comparing components across
different layers.

Computing $\eta_\ell$ is efficient because it only requires the trace of the
empirical Fisher, not the full matrix. The trace is the sum of diagonal Fisher
entries and can be estimated from squared calibration gradients:
{\small
\begin{equation}
\mathrm{Tr}(F_\ell)
=
\sum_j [F_\ell]_{j,j}
=
\sum_j
\mathbb{E}\!\left[
\left(\nabla_{W_{\ell,j}}\mathcal{L}\right)^2
\right]
\approx
\frac{1}{N}
\sum_{n=1}^{N}
\sum_j
\left(\nabla_{W_{\ell,j}}\mathcal{L}^{(n)}\right)^2
\label{eq:fisher-trace}
\end{equation}}

Meanwhile, the K-FAC trace is available from its Kronecker factors as
$\mathrm{Tr}(K_\ell)=\mathrm{Tr}(G_\ell)\mathrm{Tr}(X_\ell)$.
For the diagnostic analysis, we instantiate the above ratio on each Q-projection
head. Specifically, for the $h$-th Q head in layer $\ell$, we compute
$\eta^Q_{\ell,h}$ by applying Eq.~\ref{eq:eta-definition} to the corresponding
head weight block.

Empirically, we observe substantial variation in $\eta^Q_{\ell,h}$ across
Q-projection heads and layers of LLaVA-v1.5-7B. This indicates that different Q-head blocks are not calibrated to the same empirical-Fisher loss scale under the K-FAC surrogate. Consequently, two singular components with the same
K-FAC-based truncation loss $\frac{1}{2}\sigma_{\ell,h,i}^{2}$ may correspond
to different empirical-Fisher loss changes when they belong to different layers
or heads. This scale mismatch makes K-FAC singular values alone an unreliable
ranking criterion for cross-layer rank allocation.

Motivated by this observation, we extend the Importance Score~\cite{wang2025qsvd} to the loss-aware SVD scenario for loss-aware cross-layer rank allocation. Instead of relying on the K-FAC surrogate to compare singular values across layers, we directly use calibration gradients to estimate an empirical-Fisher-based loss sensitivity for each singular value. This provides a more loss-aware and better calibrated criterion for global rank allocation. Recall that the curvature-weighted matrix is decomposed as $\widetilde{W}=S_xWS_g=U\Sigma V^{\top}$. For the $i$-th singular value of layer $\ell$, we define its Importance Score:
{\small
\begin{equation}
\widehat{I}_{\sigma_{\ell,i}}
=
\frac{1}{N}
\sum_{n=1}^{N}
\sigma_{\ell,i}^{2}
\left[
U_{\ell}^{\top}
S_{x,\ell}^{-\top}
G_{W_\ell}^{(n)}
S_{g,\ell}^{-\top}
V_{\ell}
\right]_{i,i}^{2}
\end{equation}}
where $G_{W_\ell}^{(n)}=\nabla_{W_\ell}\ell^{(n)}$ denotes the weight
gradient of layer $\ell$ on the $n$-th calibration sample. Intuitively, this
score measures not only the reconstruction energy of each singular value,
captured by $\sigma_{\ell,i}^{2}$, but also how strongly this component is
aligned with the loss gradient after mapping the curvature-weighted SVD basis
back to the original parameter space. We then perform global rank allocation by
retaining the singular values with the largest
$\widehat{I}_{\sigma_{\ell,i}}$ under the target parameter budget.

\subsection{Low-rank Approximation for Low-precision Feed-Forward Networks}
%\subsubsection{Mixed Quantization/SVD for Feed-Forward Networks}
\label{sec:mix-quant-svd}

While Sections~\ref{sec:loss-aware-svd} and~\ref{sec:rank-alloc} focus on optimizing self-attention (SA) layers, this section extends the discussion to gated feed-forward networks (FFNs). FFN layers account for a large fraction of transformer parameters, but applying the same low-rank compression strategy uniformly to all FFN hidden channels can cause substantial accuracy degradation. Empirically, we find that decomposing the entire FFN weight matrix with SVD often introduces excessive deviation from the original model. To address this, we apply low-rank SVD only to selected FFN submatrices and introduce an iterative procedure to identify SVD-friendly hidden channels. Afterward, we further quantize the resulting matrices to reduce the computational cost and parameter size of the FFN layers.

%Some channels are better suited to low-rank decomposition, while others tolerate direct round-to-nearest (RTN) quantization. We therefore assign each hidden channel to either an SVD branch or an RTN branch, and then permute the selected channels into contiguous blocks to enable efficient hybrid execution.


%We propose an SVD-aware hybrid compression scheme for gated feed-forward
%networks (FFNs). FFN layers contain a large fraction of transformer parameters,
%yet applying a uniform compression operator to all hidden channels can be
%suboptimal: some channels are better preserved by low-rank decomposition, while
%others are more robust to direct quantization. Our goal is to assign hidden
%channels to either a low-rank SVD branch or a round-to-nearest (RTN) branch, and
%then permute the assigned channels into contiguous blocks for efficient hybrid
%execution.
Let $W_G,W_U\in\mathbb{R}^{d_{\mathrm{in}}\times m_{\mathrm{ffn}}}$ and $W_D\in\mathbb{R}^{m_{\mathrm{ffn}}\times d_{\mathrm{out}}}$ denote the gate, up, and down projection matrices, respectively, where $m_{\mathrm{ffn}}$ is the FFN hidden dimension. Given calibration inputs $X_{\mathrm{ffn}}\in\mathbb{R}^{N\times d_{\mathrm{in}}}$, with each row representing one calibration sample, the full-precision FFN output is:
{\small
\begin{equation}
Y_{\mathrm{ref}}
=
\left(
\mathrm{SiLU}(X_{\mathrm{ffn}}W_G)
\odot
X_{\mathrm{ffn}}W_U
\right)W_D
\end{equation}}





Consider the gate, up, and down projections
$W_G,W_U\in\mathbb{R}^{d_{\mathrm{in}}\times m_{\mathrm{ffn}}}$ and
$W_D\in\mathbb{R}^{m_{\mathrm{ffn}}\times d_{\mathrm{out}}}$, where
$m_{\mathrm{ffn}}$ is the FFN hidden dimension. Given calibration FFN inputs
$X_{\mathrm{ffn}}\in\mathbb{R}^{N\times d_{\mathrm{in}}}$, with each row
corresponding to one calibration sample, the full-precision FFN output is
{\small
\begin{equation}
Y_{\mathrm{ref}}
=
\left(
\mathrm{SiLU}(X_{\mathrm{ffn}}W_G)
\odot
X_{\mathrm{ffn}}W_U
\right)W_D
\end{equation}}
This channel-level assignment is well-defined because both
$\mathrm{SiLU}(\cdot)$ and the element-wise product act independently along the
hidden dimension before the down projection. Hence, hidden channel $i$ depends
only on the column pair $(W_G[:,i],W_U[:,i])$ and contributes to the output
through the row $W_D[i,:]$.

Let $\rho_{\mathrm{ffn}}$ be the target SVD-channel ratio. We allocate
$m_{\mathrm{S}}=\lfloor \rho_{\mathrm{ffn}}m_{\mathrm{ffn}}\rfloor$ channels to
the SVD branch and $m_{\mathrm{R}}=m_{\mathrm{ffn}}-m_{\mathrm{S}}$ channels to
the RTN branch. The SVD rank is set to
$r_{\mathrm{ffn}}=\lfloor \gamma_{\mathrm{ffn}}\min(d_{\mathrm{in}},m_{\mathrm{S}})\rfloor$,
where $\gamma_{\mathrm{ffn}}$ is the rank ratio. The selection starts from an
all-SVD baseline rather than an all-RTN baseline. We first simulate the quantized low-rank factorized path for $W_G$ and $W_U$ to
obtain $Z_{\mathrm{S}}$ and $Y_{\mathrm{S}}$, and also simulate the direct RTN
path to obtain $Z_{\mathrm{R}}$. Replacing channel $i$ from SVD to RTN induces
the hidden-state change
$\Delta z_i=Z_{\mathrm{R}}[:,i]-Z_{\mathrm{S}}[:,i]$.

To reduce search cost, channels are first ordered by a lightweight SVD-vs-RTN
proxy. The proxy compares the estimated RTN error and SVD residual of
$W_G[:,i]$ and $W_U[:,i]$, weighted by the magnitude of the downstream row
$W_D[i,:]$. Thus, channels whose RTN replacement is expected to be less harmful
than SVD, after accounting for their contribution through $W_D$, are evaluated
earlier.

The final assignment is obtained by greedy output-space error minimization. We
initialize $Y_{\mathrm{cur}}=Y_{\mathrm{S}}$, define
$E=Y_{\mathrm{cur}}-Y_{\mathrm{ref}}$, and cache
$M=EW_D^\top\in\mathbb{R}^{N\times m_{\mathrm{ffn}}}$. Replacing channel $i$ changes the output by the rank-one term $\Delta z_i W_D[i,:]$. Therefore, the
trial calibration MSE can be evaluated as
{\small
\begin{equation}
\mathrm{MSE}_{\mathrm{trial}}
=
\mathrm{MSE}_{\mathrm{cur}}
+
\frac{2}{N d_{\mathrm{out}}}\Delta z_i^\top M[:,i]
+
\frac{\|\Delta z_i\|_2^2\|W_D[i,:]\|_2^2}{N d_{\mathrm{out}}}.
\end{equation}}
Channel $i$ is accepted into the RTN branch only if this update decreases the
calibration MSE. Once accepted, we update
$M\leftarrow M+\Delta z_i(W_D[i,:]W_D^\top)$, avoiding full FFN re-evaluation
during the greedy search. The first $m_{\mathrm{R}}$ accepted channels form the
RTN index set $\mathcal{I}_{\mathrm{R}}$, and the SVD index set is its
complement
$\mathcal{I}_{\mathrm{S}}=\{0,\ldots,m_{\mathrm{ffn}}-1\}\setminus
\mathcal{I}_{\mathrm{R}}$. Therefore, the SVD branch consists of the channels
that remain after greedy RTN replacement, rather than the first
$m_{\mathrm{S}}$ channels in the proxy order.

After assignment, we permute the hidden channels so that the SVD and RTN
channels form contiguous blocks. Let
$\pi=[\mathrm{sort}(\mathcal{I}_{\mathrm{S}}),
\mathrm{sort}(\mathcal{I}_{\mathrm{R}})]$, and let $P_\pi$ be the corresponding
permutation matrix such that right-multiplication by $P_\pi$ reorders
hidden-channel columns according to $\pi$. The gate and up projections are
column-permuted, while the down projection is row-permuted. This permutation
preserves the FFN function: if
$Z=\mathrm{SiLU}(X_{\mathrm{ffn}}W_G)\odot X_{\mathrm{ffn}}W_U$ denotes the
original FFN hidden activation, then the permuted hidden activation is
$Z'=ZP_\pi$, and
{\small
\begin{equation}
W_G'=W_GP_\pi,\qquad
W_U'=W_UP_\pi,\qquad
W_D'=P_\pi^\top W_D,
\qquad
Z'W_D'
=
ZP_\pi P_\pi^\top W_D
=
ZW_D
\end{equation}}
Thus, the permutation only reorders hidden channels and does not change the FFN
semantics.
The hybrid branch is constructed after permutation. We split the permuted
weights by hidden-channel blocks:
$W_G'=[W_{G,\mathrm{S}}',W_{G,\mathrm{R}}']$,
$W_U'=[W_{U,\mathrm{S}}',W_{U,\mathrm{R}}']$, and
$W_D'=\begin{bmatrix} W_{D,\mathrm{S}}' \\ W_{D,\mathrm{R}}' \end{bmatrix}$,
where the SVD blocks contain the leading $m_{\mathrm{S}}$ hidden channels. The
SVD blocks $W_{G,\mathrm{S}}'$ and $W_{U,\mathrm{S}}'$ are factorized and
executed by the low-rank branch, while the RTN blocks
$W_{G,\mathrm{R}}'$ and $W_{U,\mathrm{R}}'$ are compressed by direct RTN
quantization. Let $G_{\mathrm{S}}'$ and $U_{\mathrm{S}}'$ denote the gate and up
activations produced by the low-rank SVD branch, and let $G_{\mathrm{R}}'$ and
$U_{\mathrm{R}}'$ denote those produced by the RTN branch. The output of the
hybrid FFN is:
{\small
\begin{equation}
Z_{\mathrm{hyb}}
=
\left[
\mathrm{SiLU}(G_{\mathrm{S}}')\odot U_{\mathrm{S}}',
\,
\mathrm{SiLU}(G_{\mathrm{R}}')\odot U_{\mathrm{R}}'
\right],
\qquad
Y_{\mathrm{hyb}}=Z_{\mathrm{hyb}}W_D
\end{equation}}
where the primed activations are computed from the corresponding contiguous SVD
and RTN channel blocks. When activation-aware SVD is enabled, we estimate the
FFN input covariance from $X_{\mathrm{ffn}}$, perform SVD in the whitened input
space, and absorb the inverse whitening transform into the right factor, so that the deployed low-rank factors still operate on the original FFN input space.


Under the K-FAC loss surrogate in Approximation~\ref{prop:kfac-loss-surrogate},
the loss-aware rank-$r$ approximation is given by:
{\small
\begin{equation}
\widehat W_r^{\star}
=
\arg\min_{\operatorname{rank}(\widehat W_r)\le r}
\left\|S_x(W-\widehat W_r)S_g\right\|_F^2
\label{eq:loss-aware-svd-objective}
\end{equation}
}
Let $\widetilde W=S_xWS_g$. Its SVD is written as:
{\small
\begin{equation}
\begin{gathered}
\widetilde W
=
U\Sigma V^{\top},
\qquad
\Sigma=\operatorname{diag}(\sigma_1,\ldots,\sigma_q), \\
\sigma_1\ge\cdots\ge\sigma_q\ge0,
\qquad
q=\min\{m,n\}
\end{gathered}
\label{eq:weighted-matrix-svd}
\end{equation}
}
Then the optimal rank-$r$ approximation is obtained by truncating the SVD of $\widetilde W$
and mapping it back to the original weight space:
{\small
\setlength{\jot}{1pt}
\begin{align}
\widehat W_r^{\star}
&=
S_x^{-1}U_r\Sigma_rV_r^{\top}S_g^{-1}
=
A_rB_r,
\notag\\[-0.5mm]
A_r
&=
S_x^{-1}U_r\Sigma_r^{1/2},
\qquad
B_r=
\Sigma_r^{1/2}V_r^{\top}S_g^{-1},
\label{eq:loss-aware-svd-solution}\\[-0.5mm]
\Delta\mathcal{L}_r
&\approx
\frac{1}{2} \left\|S_x(W-\widehat W_r^{\star})S_g\right\|_F^2= \frac{1}{2}
\sum_{i=r+1}^{q}\sigma_i^2
\label{eq:loss-aware-tail-loss}
\end{align}
}
\end{theorem}

\begin{proof}
Let $\Delta W=\widehat W_r-W$. From
Proposition~\ref{prop:kfac-loss-surrogate}, the K-FAC loss surrogate is:
{\small
\begin{equation}
\Delta\mathcal{L}
\approx
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
(G\otimes X)
\mathrm{vec}(\Delta W)
\label{eq:kfac-surrogate-in-proof}
\end{equation}
}
Using $X=S_x^{\top}S_x$ and $G=S_gS_g^{\top}$, together with the identities of Kronecker product
$(A\otimes B)(C\otimes D)=(AC)\otimes(BD)$ and
$\mathrm{vec}(ABC)=(C^{\top}\otimes A)\mathrm{vec}(B)$, we have:
{\small
\begin{equation}
\begin{aligned}
\Delta\mathcal{L}
&\approx
\frac{1}{2}\mathrm{vec}(\Delta W)^{\top}
(G\otimes X)
\mathrm{vec}(\Delta W) 
=
\frac{1}{2}\mathrm{vec}(\Delta W)^{\top}
(S_gS_g^{\top}\otimes S_x^{\top}S_x)
\mathrm{vec}(\Delta W) \\
&=
\frac{1}{2}\mathrm{vec}(\Delta W)^{\top}
(S_g\otimes S_x^{\top})(S_g^{\top}\otimes S_x)
\mathrm{vec}(\Delta W) 
=
\frac{1}{2}\left\|
(S_g^{\top}\otimes S_x)\mathrm{vec}(\Delta W)
\right\|_2^2 \\
&=
\frac{1}{2}\left\|
\mathrm{vec}(S_x\Delta W S_g)
\right\|_2^2
=
\frac{1}{2}\left\|
S_x\Delta W S_g
\right\|_F^2
\end{aligned}
\label{eq:kfac-to-weighted-frobenius}
\end{equation}
}

Therefore, minimizing the K-FAC surrogate is equivalent to minimizing
$\|S_x(\widehat W_r-W)S_g\|_F^2$. Since the Frobenius norm is invariant to a
global sign change, this gives the weighted low-rank objective in
Eq.~\ref{eq:loss-aware-svd-objective}.
Next, define the transformed weight and approximation as
$\widetilde W=S_xWS_g$ and $\widetilde W_r=S_x\widehat W_rS_g$. Since $S_x$
and $S_g$ are nonsingular, this transformation is one-to-one and preserves rank:
$\operatorname{rank}(\widetilde W_r)=\operatorname{rank}(\widehat W_r)$. Hence,
Eq.~\ref{eq:loss-aware-svd-objective} is equivalent to the standard rank-$r$
approximation problem:
{\small
\begin{equation}
\min_{\operatorname{rank}(\widetilde W_r)\le r}
\left\|
\widetilde W-\widetilde W_r
\right\|_F^2
\label{eq:transformed-low-rank-problem}
\end{equation}
}

By the Eckart--Young--Mirsky theorem~\cite{eckart1936approximation,mirsky1960symmetric},
the optimal solution is obtained by truncating the SVD of
$\widetilde W=U\Sigma V^{\top}$:
{\small
\begin{equation}
\widetilde W_r^{\star}=U_r\Sigma_rV_r^{\top}
\label{eq:optimal-transformed-svd}
\end{equation}
}

Mapping this solution back to the original weight space gives
$\widehat W_r^{\star}=S_x^{-1}\widetilde W_r^{\star}S_g^{-1}
=S_x^{-1}U_r\Sigma_rV_r^{\top}S_g^{-1}$. Splitting the middle singular-value
matrix symmetrically yields the deployable factorization
$A_r=S_x^{-1}U_r\Sigma_r^{1/2}$ and
$B_r=\Sigma_r^{1/2}V_r^{\top}S_g^{-1}$, which proves
Eq.~\ref{eq:loss-aware-svd-solution}.

Finally, the optimal residual in the transformed space is
$\|\widetilde W-\widetilde W_r^{\star}\|_F^2
=\sum_{i=r+1}^{q}\sigma_i^2$. Combining this residual with the factor
$\frac{1}{2}$ in the K-FAC loss surrogate gives
Eq.~\ref{eq:loss-aware-tail-loss}.
\end{proof}

\begin{proof} \textcolor{blue}{move to appendix}
For any square matrix $C$ and isotropic direction $u$ satisfying
$\mathbb{E}[uu^\top]=I/d_\ell$,
{\small
\begin{equation}
\mathbb{E}_{u}\!\left[(au)^\top C(au)\right]
=
a^2\operatorname{Tr}\!\left(C\mathbb{E}[uu^\top]\right)
=
\frac{a^2}{d_\ell}\operatorname{Tr}(C).
\label{eq:isotropic-trace-identity}
\end{equation}
}
Applying Eq.~\ref{eq:isotropic-trace-identity} to $C=F_\ell-K_\ell$ and
$C=K_\ell$ gives:
{\small
\begin{equation}
\frac{
\mathbb{E}_{u}\!\left[\frac{1}{2}(au)^\top(F_\ell-K_\ell)(au)\right]
}{
\mathbb{E}_{u}\!\left[\frac{1}{2}(au)^\top K_\ell(au)\right]
}
=
\frac{a^2\operatorname{Tr}(F_\ell-K_\ell)/d_l}
{a^2\operatorname{Tr}(K_\ell)/d_l}
=
\frac{\operatorname{Tr}(F_\ell-K_\ell)}
{\operatorname{Tr}(K_\ell)}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(K_\ell)}-1
\end{equation}
}
Finally, using $K_\ell=G_\ell\otimes X_\ell$ and
$\operatorname{Tr}(A\otimes B)=\operatorname{Tr}(A)\operatorname{Tr}(B)$ yields
Eq.~\ref{eq:eta-diagnostic}.
\end{proof}

For a discarded singular component with
$z_{\ell,i}=\operatorname{vec}(\Delta W_{\ell,i}^{\mathrm{drop}})$, the
empirical-Fisher second-order loss can be decomposed into the K-FAC prediction
and its residual:
{\small
\begin{equation}
\Delta\mathcal{L}^{F}_{\ell,i}
\approx
\frac{1}{2}z_{\ell,i}^{\top}K_\ell z_{\ell,i}
+
\frac{1}{2}z_{\ell,i}^{\top}(F_\ell-K_\ell)z_{\ell,i}
\triangleq
T^{\mathrm{KFAC}}_{\ell,i}
+
T^{\mathrm{res}}_{\ell,i}.
\label{eq:fisher-kfac-decomp}
\end{equation}
}

By Theorem~\ref{thm:loss-aware-svd},
$T^{\mathrm{KFAC}}_{\ell,i}
=\frac{1}{2}\|S_{x,\ell}\Delta W_{\ell,i}^{\mathrm{drop}}S_{g,\ell}\|_F^2
=\frac{1}{2}\sigma_{\ell,i}^2$. Thus, $\sigma_{\ell,i}^2$ measures the
K-FAC-predicted contribution of discarding the $i$-th singular component, while
$T^{\mathrm{res}}_{\ell,i}$ captures the curvature error caused by replacing
$F_\ell$ with $K_\ell$.

Proposition~\ref{prop:kfac-scale-diagnostic} shows that $\eta_\ell$ is an
average scale diagnostic for this residual. Specifically, $\eta_\ell>1$ means
that K-FAC underestimates the direction-averaged empirical-Fisher curvature of
layer $\ell$, while $\eta_\ell<1$ means that it overestimates it. Since
$\eta_\ell$ is averaged over isotropic perturbation directions, it is not a
per-component correction for $T^{\mathrm{res}}_{\ell,i}$. Instead, large
variation in $\eta_\ell$ indicates that K-FAC singular values are not reliably
calibrated for cross-layer rank allocation.

The diagnostic is inexpensive because it only requires trace statistics:
{\small
\begin{equation}
\begin{aligned}
\operatorname{Tr}(F_\ell)
&=
\operatorname{Tr}(F_{\ell,diag})
=
\sum_j
\mathbb{E}\!\left[
(\nabla_{W_{\ell,j}}\ell)^2
\right]
\approx
\frac{1}{N}
\sum_{n=1}^{N}
\left\|
\nabla_{W_\ell}\ell^{(n)}
\right\|_F^2,
\\[-0.5mm]
\operatorname{Tr}(K_\ell)
&=
\operatorname{Tr}(G_\ell\otimes X_\ell)
=
\operatorname{Tr}(G_\ell)\operatorname{Tr}(X_\ell)
\end{aligned}
\label{eq:trace-estimation}
\end{equation}
}

In our diagnostic analysis, we instantiate Eq.~\ref{eq:eta-diagnostic} on each
Q-projection head. For the $h$-th Q head in layer $\ell$, we compute $\eta^{Q}_{\ell,h}$ using the corresponding head weight block. The variation of $\eta^{Q}_{\ell,h}$ across heads and layers motivates replacing K-FAC-only ranking with an empirical-Fisher importance score.

we directly estimate the empirical-Fisher sensitivity of
removing each component. Recall that the curvature-weighted matrix of layer
$\ell$ is
$\widetilde W_\ell=S_{x,\ell}W_\ell S_{g,\ell}
=U_\ell\Sigma_\ell V_\ell^\top$. Dropping the $i$-th singular component induces
the original-space perturbation
{\small
\begin{equation}
\Delta W_{\ell,i}^{\mathrm{drop}}
=
-\sigma_{\ell,i}
S_{x,\ell}^{-1}
u_{\ell,i}v_{\ell,i}^{\top}
S_{g,\ell}^{-1}
\label{eq:singular-component-drop}
\end{equation}
}
where $u_{\ell,i}$ and $v_{\ell,i}$ are the corresponding left and right
singular vectors. Let
$\mathcal{G}_{\ell}^{(n)}=\nabla_{W_\ell}\ell^{(n)}$ be the calibration gradient
of layer $\ell$ on sample $n$. We define the empirical-Fisher importance score as
{\small
\begin{equation}
\widehat{\mathcal{I}}_{\ell,i}
=
\frac{1}{2N}
\sum_{n=1}^{N}
\left\langle
\mathcal{G}_{\ell}^{(n)},
\Delta W_{\ell,i}^{\mathrm{drop}}
\right\rangle^2
=
\frac{\sigma_{\ell,i}^{2}}{2N}
\sum_{n=1}^{N}
\left[
U_\ell^{\top}
S_{x,\ell}^{-\top}
\mathcal{G}_{\ell}^{(n)}
S_{g,\ell}^{-\top}
V_\ell
\right]_{i,i}^{2}
\label{eq:empirical-fisher-importance}
\end{equation}
}

The common factor $\frac{1}{2}$ can be omitted in implementation because it does
not affect ranking. Unlike $\sigma_{\ell,i}^2$, this score estimates the
empirical-Fisher loss sensitivity of each singular component after mapping the
curvature-weighted SVD basis back to the original parameter space.

Theorem~\ref{thm:loss-aware-svd} gives a direct implementation rule: perform SVD
in the transformed weight space and then map the truncated approximation back. %More explicitly, if $\Sigma=\operatorname{diag}(\sigma_1,\ldots,\sigma_q)$ with $\sigma_1\ge\cdots\ge\sigma_q\ge0$ and $q=\min\{m,n\}$, then $\widetilde W_r^{\star}=U_r\Sigma_rV_r^{\top}$. 
The resulting compressed weight can be implemented as a product of two low-rank factors:
{\small
\begin{equation}
\widehat W_r^{\star}
=
S_x^{-1}U_r\Sigma_rV_r^{\top}S_g^{-1}
=
A_rB_r,
\qquad
A_r=S_x^{-1}U_r\Sigma_r^{1/2},
\quad
B_r=\Sigma_r^{1/2}V_r^{\top}S_g^{-1}
\label{eq:loss-aware-svd-solution}
\end{equation}
}

The corresponding truncation loss is:
{\small
$
\Delta\mathcal{L}_r
\approx
\frac{1}{2}
\left\|S_x(W-\widehat W_r^{\star})S_g\right\|_F^2
=
\frac{1}{2}\sum_{i=r+1}^{q}\sigma_i^2
\label{eq:loss-aware-tail-loss}
$}.
In practice, $S_x$ and $S_g$ are computed from the covariance factors, with standard diagonal damping for numerical stability, via Cholesky factorization~\cite{higham1990analysis} or eigendecomposition~\cite{abdi2007eigen}. In deployment, we do not materialize $\widehat W_r^{\star}\in\mathbb{R}^{m\times n}$.
Instead, the dense operation $xW$ is replaced by the factorized computation
$xA_rB_r$, where $A_r\in\mathbb{R}^{m\times r}$ and
$B_r\in\mathbb{R}^{r\times n}$. This reduces the parameter count and dominant
MAC cost from $mn$ to $r(m+n)$. We denote the corresponding compression ratio by:
{\small
\begin{equation}
\rho_1
=
\frac{\alpha_{\mathrm{svd}}}{\alpha_{\mathrm{dense}}}
=
\frac{r(m+n)}{mn}
\label{eq:svd-param-mac-ratio}
\end{equation}
}

Thus, the factorized layer is more efficient than the dense layer when $\rho_1<1$, equivalently $r<mn/(m+n)$.


Theorem~\ref{thm:loss-aware-svd} provides a closed-form estimate of the K-FAC-based truncation loss for each curvature-weighted matrix. However, using these estimates for cross-layer comparison assumes that the layer-wise K-FAC surrogates are calibrated to a common empirical loss scale. This assumption may not hold, since K-FAC provides a local approximation within each layer rather than a globally calibrated curvature measure. We therefore first introduce a simple \textit{trace-based diagnostic} to measure the scale mismatch
between the empirical Fisher curvature and its K-FAC approximation. \textcolor{blue}{The derivation and discussion of this diagnostic are provided in Appendix~\ref{sec:appx-scale-diag}.} (\textcolor{red}{hard to follow})

\begin{proposition}[K-FAC scale diagnostic]
\label{prop:kfac-scale-diagnostic}
For layer $\ell$, let $F_\ell$ be the empirical Fisher block and $K_\ell=G_\ell\otimes X_\ell$ be its K-FAC approximation. Define the K-FAC scale diagnostic for layer $\ell$: \textcolor{red}{meaning things to proove}
{\small
\begin{equation}
\eta_\ell
\triangleq
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(K_\ell)}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(G_\ell\otimes X_\ell)}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(G_\ell)\operatorname{Tr}(X_\ell)}
\label{eq:eta-diagnostic}
\end{equation}
}
\end{proposition}

The diagnostic $\eta_\ell$ measures whether the K-FAC surrogate is globally under- or over-scaled for a layer: $\eta_\ell>1$ indicates that K-FAC underestimates the average empirical-Fisher curvature, while $\eta_\ell<1$ indicates overestimation. Therefore, large variation in $\eta_\ell$ suggests that the K-FAC singular values $\sigma_{\ell,i}^2$ are not directly comparable across layers for global rank
allocation. Importantly, $\eta_\ell$ is only a layer-level average scale diagnostic, not a correction for individual singular components. 

In our analysis, we compute this ratio for each Q-projection head. For the $h$-th Q head in layer $\ell$, we evaluate $\eta_{\ell,h}$ on the corresponding head-wise weight block. As shown in Fig.~\ref{fig:eta-diagnostic}, $\eta_{\ell,h}$ is not close to a constant scale across the model. Although some heads remain near $\eta=1$, some others show much larger deviations, with values exceeding $2$ and approaching $3$ in several layers. The mismatch also differs
across heads within the same layer. Therefore,
although $\sigma_{\ell,i}^2$ remains a meaningful local truncation-loss estimate within Assumption~\ref{assm:kfac-loss-surrogate}, it may not provide a reliable basis for comparing singular values globally across layers and heads, motivating an empirical-Fisher importance score for more accurate global rank allocation.

\textbf{Fused kernel motivation.}
As shown in Fig.~\ref{fig:mixffn_kernel}(a), the standard PyTorch implementation of FFN is bottlenecked by multiple kernel launches and repeated memory load/store operations across gate, up, and SwiGLU computations. These redundant memory accesses dominate runtime, especially under low-precision settings. To address this, we design a fused Triton kernel for MixFFN that streams data through linear projections and nonlinearities in a single pass, significantly reducing memory traffic and kernel launch overhead.


\textbf{Fused gate/up projections.}
We first fuse the gate and up projections for both SVD and dense branches.

For the SVD branch, recall that $W_{G,S}' \approx A_G B_G$ and $W_{U,S}' \approx A_U B_U$. We fuse the shared input-side projections by computing $X A_G$ and $X A_U$ jointly, producing intermediate latent representations (denoted as $L_G$ and $L_U$ in Fig.~\ref{fig:mixffn_kernel}(c)). This avoids loading $X$ multiple times. Since the second-stage projections $B_G$ and $B_U$ operate on different latent inputs, they are computed separately.

For the dense branch in Fig.~\ref{fig:mixffn_kernel}(b), we apply the same fusion strategy to $W_{G,D}'$ and $W_{U,D}'$, computing the gate and up projections in a single kernel to maximize data reuse.

\textbf{Fused SwiGLU computation.}
After projection, the SVD and dense branches are partitioned along the output dimension, consistent with the channel split in Section~\ref{sec:mix-quant-svd}. Because the same channel assignment is used for both $W_G'$ and $W_U'$, the SwiGLU operation can be applied independently within each branch without cross-branch synchronization. 

Specifically, the intermediate activations are fused through the SwiGLU operation (SiLU followed by element-wise multiplication) directly after projection, without materializing full intermediate tensors. The outputs from the SVD and dense branches are then concatenated to form the final FFN activation.

\textbf{Quantization Kernels.}
While quantization of both weights and activations reduces memory footprint and computation cost, naive activation quantization introduces additional overhead compared to FP16 computation. To mitigate this, we fuse the per-token maximum search required for quantization into preceding operations, as indicated by the blue nodes in Fig.~\ref{fig:mixffn_kernel}.

% This design results in three fused quantization patterns:

% \textbf{(1) RMSNormMaxQuant kernel.}
% The RMSNorm operation is fused with per-token maximum search and activation quantization. Instead of separately computing normalization, max reduction, and quantization, all steps are performed within a single pass over the data.

% \textbf{(2) DequantMaxQuant kernel (SVD latent).}
% For the SVD branch, we introduce a \texttt{dequantmax\_quant} kernel. During dequantization of intermediate latent activations (e.g., outputs of $X A_G$ and $X A_U$), the per-token maximum is computed within the same loop. This avoids additional memory reads/writes for intermediate activations. A subsequent step performs requantization to the target precision for the following low-bit matmul.

% \textbf{(3) NonLinearMaxQuant kernel (SwiGLU).}
% For nonlinear stages such as SwiGLU, we fuse the element-wise computation with max search and quantization. The SiLU activation and element-wise multiplication are computed first, followed immediately by per-token max reduction and quantization within the same kernel, avoiding intermediate storage.

\textbf{Summary.}
By fusing projection, nonlinear, and quantization operations, the MixFFN kernel minimizes memory movement and kernel launches. The resulting pipeline enables efficient low-precision FFN inference while maintaining functional equivalence to the original full-precision implementation. A pseudocode description of the full MixFFN pipeline is provided in the appendix.

While Sections~\ref{sec:loss-aware-svd}--\ref{sec:rank-alloc} focus on
self-attention layers, this section extends low-rank compression to gated
feed-forward networks (FFNs). FFNs contain a large fraction of transformer
parameters, but uniformly decomposing all FFN hidden channels can cause
substantial accuracy degradation. We therefore apply SVD only to selected
SVD-friendly channels and keep the remaining channels in a dense form before
low-precision quantization.

Concretely, we first compute a temporary truncated SVD for $W_G$ and $W_U$ and
use the reconstruction error to estimate how well each hidden channel can be
represented by low-rank factors. For each hidden channel, we sum the gate and up
column reconstruction errors, select the lowest-error channels as $I_S$ for the
SVD-factorized branch, and assign the remaining channels to $I_D$ for the dense
branch. Since SwiGLU multiplies gate and up activations channel-wise, the same
channel assignment is used for $W_G$ and $W_U$, and the corresponding rows of
$W_D$ are kept aligned.

To make the selected channels contiguous, we apply a shared permutation
$\pi=[\operatorname{sort}(I_S),\operatorname{sort}(I_D)]$ and define
$W'_G=W_GP_\pi$, $W'_U=W_UP_\pi$, and $W'_D=P_\pi^{\top}W_D$. This re-indexing
preserves the FFN output:
{\small
\begin{equation}
\left(\mathrm{SiLU}(xW'_G)\odot xW'_U\right)W'_D
=
\left(\mathrm{SiLU}(xW_G)\odot xW_U\right)W_D .
\end{equation}
}
The shared permutation preserves the gate/up correspondence, while the inverse
permutation on $W_D$ cancels the hidden-channel re-indexing. Since
$P_\pi^{\top}P_\pi=I$, the permutation also preserves rank, Frobenius norm, and
singular values. Thus, it does not make the FFN more low-rank; it only places
the selected channels into a contiguous block for structured factorization.

After permutation, we write
$W'_G=[W'_{G,S}\; W'_{G,D}]$ and
$W'_U=[W'_{U,S}\; W'_{U,D}]$. We recompute SVD only on the selected blocks,
$W'_{G,S}\approx A_GB_G$ and $W'_{U,S}\approx A_UB_U$, while keeping the
$I_D$ channels dense. Before RTN quantization, we insert an orthogonal rotation
between the SVD factors, $AB=(AR)(R^{\top}B)$ with $R^{\top}R=I$. This preserves
the low-rank product while improving the quantization robustness of the factors.
Finally, the rotated SVD factors, dense gate/up channels, and permuted down
projection are quantized.

Concretely, we first compute a temporary truncated SVD of $W_G$ and $W_U$ to measure how well each hidden channel can be reconstructed by SVD. For each channel, we sum the gate/up column reconstruction errors and select the lowest-error channels as $\mathcal{I}_S$ ($S$: SVD-factorized). The remaining channels form $\mathcal{I}_D$ ($D$: dense).
To apply SVD to $\mathcal{I}_S$ in a structured form, we use a grouping permutation that moves all SVD-selected channels before the dense channels. Let $\pi=\mathrm{Group}(\mathcal{I}_S,\mathcal{I}_D)$ denote this channel ordering,
where channels in $\mathcal{I}_S$ occupy the first $|\mathcal{I}_S|$ positions and channels in $\mathcal{I}_D$ occupy the remaining positions. Let $P_\pi$ be the corresponding permutation matrix. We then define permuted weight matrices $W_G'=W_GP_\pi$, $W_U'=W_UP_\pi$, and $W_D'=P_\pi^\top W_D$. Because SwiGLU multiplies gate and up activations channel-wise, the same channel assignment is used for $W_G$ and $W_U$, with the corresponding rows of $W_D$ kept aligned.
This re-indexing preserves the FFN output:
{\small
\begin{equation}
\left(\mathrm{SiLU}(xW_G')\odot xW_U'\right)W_D'
=
\left(\mathrm{SiLU}(xW_G)\odot xW_U\right)W_D
\label{eq:ffn-permutation}
\end{equation}
}

The shared permutation preserves the gate/up correspondence, while the inverse permutation on $W_D$ cancels the hidden-channel re-indexing. Since $P_\pi^\top P_\pi=I$, it also preserves rank, Frobenius norm, and singular values. Thus, the permutation does not make the full FFN more low-rank; it only arranges the selected channels into a contiguous block for structured factorization.
After permutation, we write $W_G'=[W_{G,S}'\;W_{G,D}']$ and
$W_U'=[W_{U,S}'\;W_{U,D}']$. We recompute SVD only on the selected blocks, $W_{G,S}'\approx A_GB_G$ and $W_{U,S}'\approx A_UB_U$, while keeping the $\mathcal{I}_D$ channels dense. Before RTN quantization, we insert an orthogonal rotation between the SVD factors, $AB=(AR)(R^\top B)$ with $R^\top R=I$, which preserves the low-rank product but improves factor quantization robustness. Finally, the rotated SVD factors, dense gate/up channels, and permuted down projection are RTN-quantized. In our implementation, we apply SVD to 50\% of the FFN hidden channels, compress the selected SVD branch to a parameter ratio of $\rho_1=90\%$, and skip the last five transformer layers for FFN SVD. This empirically provides a better balance between compression, acceleration, and accuracy.

==> main_pre_camera_ready.tex <==
% \documentclass{article}

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2026

% The authors should use one of these tracks.
% Before accepting by the NeurIPS conference, select one of the options below.
% 0. "default" for submission
\PassOptionsToPackage{numbers,sort&compress}{natbib}
\usepackage[main]{neurips_2026}
% the "default" option is equal to the "main" option, which is used for the Main Track with double-blind reviewing.
% 1. "main" option is used for the Main Track
%  \usepackage[main]{neurips_2026}

% After being accepted, the authors should add "final" behind the track to compile a camera-ready version.
% 1. Main Track
 % \usepackage[main, final]{neurips_2026}

% "preprint" option is used for arXiv or other preprint submissions
 % \usepackage[preprint]{neurips_2026}

% to avoid loading the natbib package, add option nonatbib:
%    \usepackage[nonatbib]{neurips_2026}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}   % \resizebox, \rotatebox
\usepackage{booktabs}   % \toprule, \midrule, \bottomrule, \cmidrule
\usepackage{multirow}   % \multirow
\usepackage{makecell}   % \makecell
\usepackage[table]{xcolor} % \cellcolor
\usepackage{tabularx}
\usepackage{wrapfig}
\usepackage{adjustbox}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\usepackage{amsthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{approximation}[theorem]{Approximation}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\usepackage{algorithm}
\usepackage{algpseudocode}

\newcommand{\accval}[1]{\fontsize{9.8pt}{10pt}\selectfont #1}

\title{LSVD: Loss-Aware Low-Rank Approximation for Efficient Low-Precision Vision-Language Models}
% LSVD: Loss-Aware Low-Rank Approximation for Fast and Efficient Execution of Low-Precision Vision-Language Models
% LA-QSVD


\author{
}


\begin{document}


\maketitle


\begin{abstract}
Vision-language models (VLMs) deliver strong multimodal reasoning capabilities, but their large computational cost and high parameter counts make deployment challenging on resource-constrained devices. Low-rank decomposition has emerged as a promising compression technique, yet existing methods often optimize local matrix reconstruction error, rely on uniform or heuristic rank allocation, and focus mainly on attention projections while leaving feed-forward networks underexplored. In this paper, we propose~\textit{LSVD}, a loss-aware low-rank approximation framework for efficient low-precision VLMs. LSVD derives a curvature-weighted SVD objective from a second-order approximation of the model loss and uses Kronecker-factored Fisher information to guide decomposition toward downstream performance rather than reconstruction alone. We further introduce a loss-aware cross-layer rank allocation strategy based on calibration gradients, enabling more effective parameter budgeting across layers. Finally, we extend low-rank compression to FFN layers through a hybrid scheme that combines SVD with quantization.
The evaluation results show that LSVD achieves more than $2.3\times$ decoding speedup over previous work while preserving strong accuracy under low-precision inference.

\end{abstract}



\section{Introduction}
\begin{wrapfigure}{r}{0.7\textwidth}
    \centering
    \vspace{-10pt}
\includegraphics[width=0.7\textwidth]{figures/overall.pdf}
    \vspace{-10pt}
    \caption{
    (a) A VLM model. (b) Overview of LSVD Framework.
    }
    \label{fig:lsvd_overall}
    \vspace{-5pt}
\end{wrapfigure}
Vision–language models (VLMs) have become an important research direction in modern AI because they bridge visual perception and language understanding. By reasoning over both image and text inputs, VLMs support a wide range of multimodal tasks, such as image captioning~\cite{hu2022scaling, li2022blip,li2023blip2, chen2022visualgpt, dzabraev2024vlrm}, visual question answering~\cite{chappuis2022prompt, bazi2023vision, bai2023qwen,wang2024surgical}, and multimodal semantic retrieval~\cite{li2024searchlvlms,sun2025leveraging}. Despite their strong performance, these models impose substantial implementation costs. Processing high-dimensional visual features together with textual context leads to intensive computation, while autoregressive decoding repeatedly accesses model states and generated tokens, creating severe memory-bandwidth pressure during inference and therefore high inference latency. On the other hand, the large size of VLMs leads to substantial storage overhead, further limiting their deployment on storage-constrained devices.


While quantization and pruning have been widely explored to reduce the computation and storage costs of large models~\cite{lin2024duquant,tseng2024quip,ashkboos2024quarot,xiang2024dfrot,wang2024qvlm}, low-rank decomposition has recently attracted increasing attention as another promising compression approach. By factorizing the query (Q), key (K), and value (V) projection matrices in self-attention blocks into low-rank components, prior studies have demonstrated notable reductions in parameter count and computational cost~\cite{wang2025svdllmv2,yuan2023asvd,wang2024svd,li2025adasvd,li2024svdqunat,chang2024palu,wang2025dobi,wang2025qsvd,wang2026wsvd}. However, several important directions remain underexplored. First, although individual optimization techniques have shown promising gains, it remains unclear whether combining them can yield further improvements. Second, rank allocation across VLM layers remains insufficiently studied, although 
different layers may exhibit distinct sensitivity to compression and therefore require non-uniform rank assignments. Finally, most existing efforts focus primarily on attention projections, while the feed-forward network (FFN) layers, which account for a large fraction of model parameters and storage cost, remain a critical but less explored target for low-rank compression.


To address these limitations, we systematically revisit low-rank compression for VLMs along these underexplored directions, and propose~\textit{Loss-Aware Low-Rank Approximation for
Efficient Low-Precision Vision-Language Models} (LSVD). Our contributions are summarized as follows:

\begin{itemize}
% \item LSVD formulates SVD under a curvature-weighted objective derived from a second-order approximation of the model loss, using Kronecker-factored Fisher information to make the decomposition better aligned with downstream VLM performance rather than only minimizing reconstruction error.
\item LSVD derives a loss-aware SVD objective from a second-order approximation of the model loss, using Kronecker-factored Fisher information to align low-rank decomposition with downstream VLM performance rather than only minimizing reconstruction error.
\item LSVD provides an analysis of why singular values obtained from loss-aware SVD are not directly comparable across layers and heads, and introduces a calibration-gradient-based importance score for more reliable global rank allocation.
\item LSVD extends low-rank compression to FFN layers through a hybrid SVD--quantization scheme that assigns each channel to the compression branch it can better tolerate.
\item We develop Triton kernels for the hybrid low-rank FFN and low-precision SA layers. The evaluation results show that LSVD achieves a decoding speedup of $4.7\times$ over Flash Decoding and $2.3\times$ over WSVD, while preserving accuracy under low-precision inference.
\end{itemize}

\section{Related Work}
\label{sec:related_work}
\paragraph{Vision-Language Model}
VLMs extend LLMs to multimodal reasoning by incorporating visual inputs into language-conditioned generation~\cite{li2022blip, li2023blip2, liu2023visual-llava, 10.5555/3666122.3668264, beyer2024paligemma, grattafiori2024llama, wang2024qwen2}. By aligning visual features with the LLM semantic space, they support image captioning, visual question answering, grounding, document understanding, and video comprehension. Modern VLMs typically consist of a vision encoder, a projection module, and an autoregressive LLM, as seen in BLIP/InstructBLIP~\cite{li2022blip, li2023blip2}, LLaVA~\cite{liu2023visual-llava}, PaLI-Gemma~\cite{beyer2024paligemma}, Qwen-VL~\cite{wang2024qwen2}, and SmolVLM~\cite{marafioti2025smolvlm}. Despite their strong capabilities, VLMs are expensive to deploy because they inherit LLM computation and memory costs while adding vision encoders and long visual-token sequences. This challenge motivates compact VLMs~\cite{yuan2023tinygpt, zhou2024tinyllava, marafioti2025smolvlm} and compression techniques such as low-rank decomposition and quantization.

%Vision--Language Models (VLMs) extend LLMs to multimodal reasoning by incorporating visual inputs into language-conditioned generation~\cite{li2022blip, li2023blip2, liu2023visual-llava, 10.5555/3666122.3668264, beyer2024paligemma, grattafiori2024llama, wang2024qwen2}. By aligning visual features with the LLM semantic space, VLMs support tasks such as image captioning, visual question answering, grounding, document understanding, and video comprehension. Modern VLMs typically use a modular architecture, where a vision encoder extracts visual tokens, a projection module maps them into the LLM embedding space, and an autoregressive LLM jointly processes visual and textual tokens. This design underlies models such as BLIP/InstructBLIP~\cite{li2022blip, li2023blip2}, LLaVA~\cite{liu2023visual-llava}, PaLI-Gemma~\cite{beyer2024paligemma}, Qwen-VL~\cite{wang2024qwen2}, and SmolVLM~\cite{marafioti2025smolvlm}. Despite their strong capabilities, VLMs remain costly to deploy because they inherit the computation and memory demands of LLMs while adding vision encoders and long visual-token sequences. This makes deployment difficult on edge and real-time systems with limited memory, bandwidth, and latency budgets, motivating compact VLMs~\cite{yuan2023tinygpt, zhou2024tinyllava, marafioti2025smolvlm} and compression techniques such as low-rank decomposition and quantization.


\paragraph{Low-Rank Approximation for Large Models}
%\label{sec:rw-lra}
Low-rank approximation is a classical approach for reducing the storage and computational cost of large matrices. A standard formulation is Singular Value Decomposition (SVD)~\cite{jolliffe2016principal}, which factorizes a weight matrix $W \in \mathbb{R}^{m \times n}$ as $W = U \Sigma V^{T}$, where $U$ and $V$ contain the left and right singular vectors, and $\Sigma$ is a diagonal matrix of singular values. Retaining only the largest $r$ singular components gives the rank-$r$ approximation: $W \approx U_r \Sigma_r V_r^{T}$,
% {\small
% \begin{equation}
% \label{eqn:low_rank_svd}
%     W \approx U_r \Sigma_r V_r^{T}
% \end{equation}}
which can be implemented as two smaller matrices, $W \approx AB$ with $A= U_r \Sigma_r^{1/2}\in \mathbb{R}^{m \times r}$ and $B=\Sigma_r^{1/2}V_r^{T} \in \mathbb{R}^{r \times n}$. When $r \ll \min(m,n)$, this decomposition reduces both parameter count and arithmetic cost.
SVD-based compression has been extensively studied for large language models and vision--language models~\cite{noach2020compressing, hsu2022language, yuan2023asvd, wang2024svd, li2024svdqunat, chang2024palu, li2025adasvd, wang2025dobi, wang2025qsvd}. While early work directly applied vanilla SVD to pretrained weights~\cite{noach2020compressing}, later methods improve robustness by incorporating calibration or sensitivity information: FWSVD~\cite{hsu2022language} uses Fisher information, ASVD~\cite{yuan2023asvd} accounts for activation outliers, and SVD-LLM~\cite{wang2024svd} and Dobi-SVD~\cite{wang2025dobi} reduce layer-wise truncation error. Recent methods further refine rank allocation~\cite{li2025adasvd, wang2025qsvd} or combine low-rank decomposition with quantization~\cite{li2024svdqunat,wang2026wsvd}.

Beyond weight compression, low-rank approximation has also been applied to inference-time memory reduction and acceleration, particularly for KV cache compression~\cite{chang2024palu, yu2024effectively,wang2026wsvd}. By decomposing the key and value projection matrices, for example $W_K \approx A_KB_K$ and $W_V \approx A_VB_V$, the cache can keep lower-dimensional latent representations $C_K = xA_K$ and $C_V = xA_V$, where $x$ denotes the input. The full keys and values are then reconstructed only when needed as $K = C_KB_K$ and $V = C_VB_V$, avoiding storage of the full-dimensional KV states. This reduces KV cache footprint and memory traffic during autoregressive decoding, which can improve decoding throughput, especially in long-context generation and multimodal models with large token budgets.

\paragraph{Quantization for Large Models}
%\label{sec:rw-quant}
Quantization reduces the memory and inference cost of large models by mapping weights and activations to low-bit formats, with post-training quantization (PTQ) being especially attractive because it avoids retraining. Representative LLM PTQ methods include GPTQ~\cite{frantar2022gptq}, AWQ~\cite{lin2024awq}, and SmoothQuant~\cite{xiao2023smoothquant}, which respectively use second-order error compensation, activation-aware channel protection, and channel-wise scaling to improve robustness. Recent methods further improve low-bit quantization through learned parameters, rotations, and optimized kernels, such as OmniQuant~\cite{shao2023omniquant}, QuaRot~\cite{ashkboos2024quarot}, SpinQuant~\cite{liu2024spinquant}, and QServe~\cite{lin2025qserve}. For VLMs, quantization is more challenging due to modality-dependent activation distributions and different sensitivities between visual and textual tokens; Q-VLM~\cite{wang2024qvlm} and MBQ~\cite{li2024mbq} address these issues through cross-layer dependency modeling and modality-balanced calibration.

\paragraph{Kronecker-Factored Approximate Curvature}
%\label{sec:rw-kfac}
Second-order curvature provides a principled way to measure parameter sensitivity, but the full Hessian or Fisher matrix is prohibitively expensive to compute and store for large models. For a linear layer with $d_{\mathrm{in}}d_{\mathrm{out}}$ parameters, the corresponding Fisher block contains $O(d_{\mathrm{in}}^2d_{\mathrm{out}}^2)$ entries. K-FAC~\cite{martens2015optimizing} makes second-order curvature tractable by approximating this block with a Kronecker product of activation and gradient covariance factors, reducing the curvature representation to two much smaller covariance matrices. For a linear layer $y=xW$ with input activation $x$ and output gradient $g$, K-FAC approximates the Fisher information: $F_W \approx \mathbb{E}[g^\top g] \otimes \mathbb{E}[x^\top x]$, 
% \begin{equation}
% F_W \approx \mathbb{E}[g^\top g] \otimes \mathbb{E}[x^\top x]
% \end{equation}
thereby retaining structured curvature information at substantially lower cost.
Originally proposed for natural-gradient optimization~\cite{martens2015optimizing}, Kronecker-factored curvature has also been used for curvature-aware compression. EigenDamage~\cite{wang2019eigendamage} performs structured pruning in the Kronecker-factored eigenbasis, and the LLM Surgeon~\cite{van2023llm} scales such approximations to large language models for pruning and weight-update compensation. In this work, we use K-FAC as a tractable approximation of local loss curvature, enabling low-rank approximation to be guided by estimated model-loss sensitivity rather than only local reconstruction error.


\section{Method}
\label{sec:method}

\subsection{Preliminary}
\label{sec:loss-aware-lra}

Conventional SVD-based low-rank approximation is usually formulated as a local
matrix reconstruction problem. Given a weight matrix $W$, truncated SVD solves
$\arg\min_{\widehat{W}: \mathrm{rank}(\widehat{W})\le r}
\|W-\widehat{W}\|_F^2$, where $\widehat{W}$ denotes the compressed weight with low rank.
Since this objective ignores the input distribution, activation-aware methods~\cite{yuan2023asvd,wang2024svd,wang2025dobi}
instead minimize layer-wise output error on calibration activations, e.g.,
$\|X(W-\widehat{W})\|_F^2$.
Other approaches further incorporate gradients or Fisher to guide
truncation and rank allocation~\cite{hsu2022language,wang2025qsvd,wang2026wsvd}.
Nevertheless, the decomposition itself remains largely driven by local reconstruction criteria rather than the end-to-end training objective. In the following sections, we therefore derive a loss-aware low-rank objective from a local curvature approximation of the model loss as illustrated in Fig.~\ref{fig:loss-aware-svd}. Following K-FAC~\cite{martens2015optimizing} and prior curvature-aware compression methods~\cite{wang2019eigendamage,van2023llm}, we approximate the loss increase caused by compression using a second-order Kronecker-factored Fisher surrogate.
The derivation from a local quadratic loss approximation is provided in Appendix~\ref{sec:appx-loss-surrogate}.

\begin{assumption}[K-FAC loss surrogate for weight compression]
\label{assm:kfac-loss-surrogate}
Consider a linear layer $y=xW$, and let
$\Delta W=\widehat{W}-W$ denote the perturbation introduced by replacing the pretrained weight $W$ with its compressed approximation $\widehat{W}$. The compression-induced loss increase is estimated by:
{\small
\begin{equation}
\Delta \mathcal{L}
\approx
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
(G\otimes X)
\mathrm{vec}(\Delta W)
\label{eq:kfac-loss-surrogate}
\end{equation}
}
where $x$ is the input activation, $g=\nabla_y\ell$ is the output gradient of the per-sample loss, and $X=\mathbb{E}[x^{\top}x]$ and $G=\mathbb{E}[g^{\top}g]$ are the two K-FAC factors estimated on the calibration set.
\end{assumption}



\subsection{Loss-Aware Singular Value Decomposition}
\label{sec:loss-aware-svd} 
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/loss_aware_svd.pdf}
    \vspace{-15pt}
    \caption{Vanilla SVD minimizes weight reconstruction error. Activation-aware SVD such as SVD-LLM~\cite{wang2024svd} reduces layer-wise output error with input activation statistics. Loss-aware SVD performs SVD in a curvature-weighted weight space to minimize the compression-induced model loss.}
    \label{fig:loss-aware-svd}
    \vspace{-13pt}
\end{figure}
Building on Assumption~\ref{assm:kfac-loss-surrogate}, we derive the low-rank approximation of a weight matrix that minimizes the estimated compression-induced loss increase. Consider a candidate linear layer with weight $W\in\mathbb{R}^{m\times n}$ and its rank-$r$ approximation $\widehat W_r$. The associated activation and gradient covariances are factorized as $X=S_x^{\top}S_x$ and $G=S_gS_g^{\top}$ with Cholesky factorization~\cite{higham1990analysis}, where $S_x$ and $S_g$ are assumed
nonsingular.

\begin{theorem}[Optimal loss-aware rank-$r$ weight approximation]
\label{thm:loss-aware-svd}
Under Assumption~\ref{assm:kfac-loss-surrogate}, define the curvature-weighted
weight matrix $\widetilde W=S_xWS_g$ and let
$\widetilde W=U\Sigma V^{\top}$ be its SVD, where
$\Sigma=\operatorname{diag}(\sigma_1,\ldots,\sigma_q)$ and
$q=\min\{m,n\}$. The rank-$r$ approximation of $W$ that minimizes the estimated compression-induced loss increase, and the corresponding truncation loss, are:
{\small
\begin{equation}
\widehat W_r^{\star}
=
S_x^{-1}U_r\Sigma_rV_r^{\top}S_g^{-1},
\qquad
\Delta\mathcal{L}_r
\approx
\frac{1}{2}\sum_{i=r+1}^{q}\sigma_i^2
\label{eq:loss-aware-svd-solution-compact}
\end{equation}
\vspace{-10pt}
}
\end{theorem}

Theorem~\ref{thm:loss-aware-svd} directly leads to an implementable procedure.
Given a calibration set, we collect the input activations $x$ and output
gradients $g$ for each candidate linear layer, and estimate
$X=\mathbb{E}[x^{\top}x]$ and $G=\mathbb{E}[g^{\top}g]$. Then we compute factors $S_x$ and $S_g$ using Cholesky factorization~\cite{higham1990analysis}, 
%either Cholesky factorization~\cite{higham1990analysis} or eigen-decomposition~\cite{abdi2007eigen},
such that $X=S_x^{\top}S_x$ and $G=S_gS_g^{\top}$. Next, we form the transformed weight $\widetilde W=S_xWS_g$, perform truncated SVD to obtain $\widetilde W_r^{\star}=U_r\Sigma_rV_r^{\top}$, and map it back as:
{\small
\begin{equation}
\widehat W_r^{\star}
=
S_x^{-1}U_r\Sigma_rV_r^{\top}S_g^{-1}
=
A_rB_r,
\qquad
A_r=S_x^{-1}U_r\Sigma_r^{1/2},
\quad
B_r=\Sigma_r^{1/2}V_r^{\top}S_g^{-1}
\label{eq:loss-aware-svd-solution}
\end{equation}
\vspace{-10pt}
}

The corresponding truncation loss is:
{\small
$
\Delta\mathcal{L}_r
\approx
\frac{1}{2}
\left\|S_x(W-\widehat W_r^{\star})S_g\right\|_F^2
=
\frac{1}{2}\sum_{i=r+1}^{q}\sigma_i^2
\label{eq:loss-aware-tail-loss}
$}.
At inference, we do not materialize
$\widehat W_r^{\star}\in\mathbb{R}^{m\times n}$; instead, we replace $xW$ with
$xA_rB_r$, where $A_r\in\mathbb{R}^{m\times r}$ and
$B_r\in\mathbb{R}^{r\times n}$. This reduces the parameter count and dominant multiply-accumulation (MAC) cost from $mn$ to $r(m+n)$, giving the compression ratio $\rho_1=\frac{r(m+n)}{mn}$. 
% {\small
% \begin{equation}
% \rho_1
% =
% \frac{r(m+n)}{mn}
% \label{eq:svd-param-mac-ratio}
% \end{equation}
% }
Thus, when $\rho_1<1$, or equivalently $r<mn/(m+n)$, the low-rank form reduces parameter count and computational cost.


\subsection{Loss-Aware Cross-Layer Rank Allocation}
\label{sec:rank-alloc}

Theorem~\ref{thm:loss-aware-svd} shows that the squared singular values of the curvature-weighted matrix estimate the loss increase caused by truncating the corresponding singular components. For layer $\ell$, let $\sigma_{\ell,i}$ denote the $i$-th singular value after loss-aware SVD. This gives a natural intuition for rank allocation: singular components with larger $\sigma_{\ell,i}^2$ should be preserved first, and
layers or heads with more large singular values should receive more ranks.
However, using these K-FAC-based singular values for global rank allocation assumes that values computed from different layers or attention heads are directly comparable. In other words, a larger $\sigma_{\ell,i}$ in one layer $\ell$ should correspond to a
larger loss increase than a smaller $\sigma_{\ell',j}$ in another layer $\ell'$. This comparability is not guaranteed in practice. K-FAC estimates curvature separately for each layer or attention head, so the loss estimate in Assumption~\ref{assm:kfac-loss-surrogate} may differ from the empirical-Fisher estimate by layer- or head-dependent scaling factors.
In this case, the same value of $\sigma_{\ell,i}$ may correspond to different loss increases in different layers or heads. Although $\sigma_{\ell,i}$ is meaningful for local truncation within the same layer or head, it may be unreliable for ranking components globally across layers and heads. 
% To examine this issue, we compare the difference of average curvature magnitude $\eta_\ell$ given by  empirical Fisher with that given by its K-FAC approximation \textcolor{blue}{for layer $\ell$} 
To examine this issue, we use the trace ratio $\eta_\ell$ between the empirical-Fisher block and its K-FAC approximation for layer $\ell$ to indicate K-FAC's estimation bias:
%(\textcolor{red}{what is $\eta_\ell, F_\ell, G_\ell, X_\ell, G_\ell$? Have you ever defined them? Why Tr(.) is used? Is it used to estimated empirical fisher score?})
{\small
\begin{equation}
\eta_\ell
\triangleq
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(K_\ell)}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(G_\ell\otimes X_\ell)}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(G_\ell)\operatorname{Tr}(X_\ell)}
\label{eq:eta-scale-ratio}
\end{equation}
}

\begin{wrapfigure}{r}{0.25\textwidth}
    \centering
    \vspace{-20pt}
    \includegraphics[width=0.25\textwidth]{figures/eta_sample.pdf}
    \vspace{-15pt}
    \caption{Values of $\eta_{\ell,h}$ across 32 layers (4 heads illustrated).}
    \label{fig:eta-diagnostic}
    \vspace{-15pt}
\end{wrapfigure}
where $F_\ell$ is the empirical-Fisher block of layer $\ell$, $K_\ell=G_\ell\otimes X_\ell$ is its K-FAC approximation, and $X_\ell$ and $G_\ell$ are the activation-side and gradient-side K-FAC factors of layer $\ell$. We provide a formal derivation of this trace ratio and its connection to the
K-FAC approximation error in Appendix~\ref{sec:appx-scale-diag}.
$\eta_\ell>1$ means that K-FAC underestimates the average curvature measured by the empirical Fisher for layer $\ell$, while $\eta_\ell<1$ means that it overestimates it. 
Large variation in $\eta_\ell$ indicates that K-FAC-based singular values are not consistently scaled across layers or heads.
We use this ratio only to expose this mismatch, rather than to rescale individual singular components. 

To empirically examine and quantify this mismatch, we analyze LLaVA-v1.5 7B~\cite{liu2023visual-llava} by computing this ratio for each Q-projection head. For the $h$-th Q head in layer $\ell$, we evaluate $\eta_{\ell,h}$ on the corresponding head-wise weight block.
As shown in Fig.~\ref{fig:eta-diagnostic}, $\eta_{\ell,h}$ varies substantially across both layers and heads. Some heads remain close to $\eta=1$, while others exceed $2$ and approach $3$ in several layers. Heads within the same layer also
show different degrees of mismatch. These results show that K-FAC-based singular values are not on a consistent scale across layers and heads, and therefore may not be directly compared for global rank allocation. This motivates our use of an empirical-Fisher importance score for more accurate component ranking.


\paragraph{Empirical-Fisher singular-value importance.}
Instead of globally ranking singular components by the K-FAC estimate $\sigma_{\ell,i}^2$, we extend the Importance Score~\cite{wang2025qsvd} to the loss-aware SVD setting. Specifically, we use calibration gradients to directly estimate the empirical-Fisher-based loss sensitivity of each singular component, providing a better calibrated and more loss-aware criterion for cross-layer rank allocation.
 Recall that %the curvature-weighted matrix is decomposed as 
$\widetilde{W}=S_xWS_g=U\Sigma V^{\top}$. For the $i$-th singular value of layer $\ell$, we define its importance score as:
{\small
\begin{equation}
\widehat{I}_{\ell,i}
=
\frac{1}{N}
\sum_{n=1}^{N}
\sigma_{\ell,i}^{2}
\left[
U_{\ell}^{\top}
S_{x,\ell}^{-\top}
G_{W_\ell}^{(n)}
S_{g,\ell}^{-\top}
V_{\ell}
\right]_{i,i}^{2}
\end{equation}}
where $G_{W_\ell}^{(n)}=\nabla_{W_\ell}\ell^{(n)}$ denotes the weight gradient of layer $\ell$ on the $n$-th calibration sample. This score measures how much each singular component contributes to the empirical-Fisher quadratic loss approximation, rather than relying on the K-FAC surrogate used to compute the SVD basis. It combines the singular value magnitude, captured by $\sigma_{\ell,i}^{2}$, with its alignment to the calibration gradients after mapping the basis back to the original parameter space. We provide the derivation in Appendix~\ref{sec:appx-importance-score}.

\paragraph{Global rank allocation.}
We allocate ranks by selecting singular components under a target parameter budget $B$. For the $\ell$-th candidate matrix $W_\ell\in\mathbb{R}^{m_\ell\times n_\ell}$, where $m_\ell$ and $n_\ell$ are its input and output dimensions, preserving one singular component will cost additional $\kappa_\ell=m_\ell+n_\ell$ parameters. Let
$\mathcal{S}$ denote the set of selected components, where
$(\ell,i)\in\mathcal{S}$ means that the $i$-th singular component of $W_\ell$ is retained. The global selection problem is:
%(\textcolor{red}{not clear, what is $B$? what is $m_{l}$, $n_{l}$, $\kappa_\ell$? Is $n$ mean $n-th$ calibration sample? what is rank-$1$? }):

\begin{equation}
\small
\mathcal{S}^{\star}
=
\arg\max_{\mathcal{S}}
\sum_{(\ell,i)\in\mathcal{S}}
\widehat{I}_{\ell,i}
\quad
\mathrm{s.t.}
\quad
\sum_{(\ell,i)\in\mathcal{S}}
\kappa_\ell
\le B
\label{eq:global-rank-allocation}
\end{equation}

The rank assigned to candidate layer $\ell$ is
$r_\ell=\left|\{i:(\ell,i)\in\mathcal{S}^{\star}\}\right|$.
If all candidate layer matrices have the same shape, the problem reduces to globally keeping the components with
the largest $\widehat{I}_{\ell,i}$. When candidate matrices have different shapes, retaining a singular component can incur different parameter costs. We therefore rank components by importance per parameter, $\widehat{I}_{\ell,i}/\kappa_\ell$, and greedily retain the highest-ranked components until the parameter budget $B$ is reached.


In LSVD, we treat the per-head QKV projections in self-attention layers as candidate matrices. We apply the loss-aware SVD from Sec.~\ref{sec:loss-aware-svd} to each per-head projection and use the proposed rank allocation strategy to assign ranks across layers and heads. This compresses QKV weights and reduces projection cost. For K/V projections, the per-head low-rank form also lowers KV-cache memory traffic during autoregressive decoding. Overall, LSVD accelerates inference while preserving accuracy by retaining the most important singular components.


\subsection{Quantization-Aware Whitening for SVD}
\label{sec:qa-whitening}
To further reduce computational cost, we apply linear quantization to both activations and low-rank weights. The loss-aware SVD objective in Sec.~\ref{sec:loss-aware-svd} uses the input-side K-FAC factor  $X=\mathbb{E}[x^{\top}x]$, which corresponds to a full-precision linear layer $y=xW$. In deployment, however, activation quantization replaces the input with $\tilde{x}=Q(x)$, where $Q(\cdot)$ is the activation quantization function with its scale and clipping range fixed after calibration. As a result, substituting $W$ with its low-rank approximation $\widehat{W}$ induces the quantized-output perturbation $\Delta y_q=\tilde{x}(\widehat{W}-W)$, rather than $x(\widehat{W}-W)$.
To align the whitening objective with the deployed low-precision layer, we adopt the~\textit{Quantization-Aware Whitening} (QAW) by estimating the input-side K-FAC factors using quantized calibration activations: $X_q=\mathbb{E}[\tilde{x}^{\top}\tilde{x}]$. We then factorize it as $X_q=S_{x,q}^{\top}S_{x,q}$ and construct the transformed weight $\widetilde W_q=S_{x,q}WS_g$. The remaining steps follow Sec.~\ref{sec:loss-aware-svd}: we perform truncated SVD on $\widetilde W_q$ and map the resulting low-rank factors back to the original weight space. After obtaining the low-rank factors, following prior work~\cite{wang2025qsvd}, we insert a rotation matrix~\cite{ashkboos2024quarot} between them before weight quantization, which preserves the low-rank product
while smoothing outliers and improving quantization robustness. When activation quantization is disabled, $Q$ reduces to the identity map, so $X_q=X$, and this formulation recovers the standard loss-aware SVD in Sec.~\ref{sec:loss-aware-svd}.  %(\textcolor{red}{should we mentioned hadamard? how the outlier is smoothed?})


\subsection{Low-rank Approximation for Low-precision Feed-Forward Networks}
\label{sec:mix-quant-svd}

% \begin{wrapfigure}{r}{0.63\linewidth}
% \vspace{-12pt}
% \begin{minipage}{0.98\linewidth}
{%\small
\begin{algorithm}[tb]
\caption{SVD-aware Hybrid FFN Compression}
\label{alg:hybrid-ffn}
\small
\begin{algorithmic}[1]
\Require FFN weights $W_G,W_U \in R^{ d_{\text{in}}\times d_\text{ffn}},W_D \in R^{ d_\text{ffn}\times d_{\text{out}}}$; SVD channel ratio $\gamma$; SVD retention ratio $\rho_{\rm ffn}$
\Ensure Quantized hybrid low-rank--dense FFN

\State $\bar W_G,\bar W_U \leftarrow
\mathrm{LowRank}(W_G;\rho_{\rm ffn}),\mathrm{LowRank}(W_U;\rho_{\rm ffn})$
\Comment{temporary SVD for channel scoring}

\For{$j=1,\ldots,d_{\rm ffn}$}
    \State $e_j \leftarrow
    \|W_G[:,j]-\bar W_G[:,j]\|_2^2
    +\|W_U[:,j]-\bar W_U[:,j]\|_2^2$
    \Comment{SVD error for each hidden channel}
\EndFor

\State $\mathcal{I}_S \leftarrow$ indices of the $\lfloor \gamma d_{\rm ffn}\rfloor$ smallest scores in $\{e_j\}$
\Comment{SVD-friendly channels}
\State $\mathcal{I}_D \leftarrow \{1,\ldots,d_{\rm ffn}\}\setminus\mathcal{I}_S$
\Comment{other channels kept dense}

\State $\pi \leftarrow \mathrm{Concat}(\mathcal{I}_S,\mathcal{I}_D)$
\Comment{new channel order with SVD channels first}
\State $P_\pi \leftarrow$ permutation matrix induced by this order
\State $W_G',W_U',W_D' \leftarrow W_GP_\pi,\; W_UP_\pi,\; P_\pi^\top W_D$
\Comment{preserve FFN output}

\State $[W_{G,S}',W_{G,D}'] \leftarrow \mathrm{Split}(W_G',|\mathcal{I}_S|)$, \quad
$[W_{U,S}',W_{U,D}'] \leftarrow \mathrm{Split}(W_U',|\mathcal{I}_S|)$
\Comment{separate SVD and dense blocks}

\State $(A_G,B_G),(A_U,B_U) \leftarrow
\mathrm{LowRank}(W_{G,S}';\rho_{\rm ffn}),\;
\mathrm{LowRank}(W_{U,S}';\rho_{\rm ffn})$
\Comment{SVD selected blocks}

\For{$T\in\{G,U\}$}
    \State $R_T \leftarrow \mathrm{Rotation}(\mathrm{rank}(A_T))$
    \Comment{orthogonal rotation: $R_T^\top R_T=I$}
    \State $(A_T,B_T) \leftarrow (A_TR_T,R_T^\top B_T)$
    \Comment{preserve product while smoothing factors}
    \State $(A_{T,q},B_{T,q}) \leftarrow \mathrm{RTN}(A_T,B_T)$
\EndFor

\State $W_{G,D,q}',W_{U,D,q}',W_{D,q}' \leftarrow
\mathrm{RTN}(W_{G,D}'),\mathrm{RTN}(W_{U,D}'),\mathrm{RTN}(W_D')$
\Comment{quantize dense branch and down projection}

\State \Return $\{A_{G,q},B_{G,q},A_{U,q},B_{U,q},
W_{G,D,q}',W_{U,D,q}',W_{D,q}'\}$
\end{algorithmic}
\end{algorithm}
% \vspace{-30pt}
}
% \end{minipage}
% \vspace{-12pt}
% \end{wrapfigure}


While Sections~\ref{sec:loss-aware-svd} and~\ref{sec:rank-alloc} focus on optimizing self-attention (SA) layers, this section extends the discussion to gated feed-forward networks (FFNs). FFN layers account for a large fraction of transformer parameters, but applying the same low-rank compression strategy uniformly to all FFN hidden channels can cause substantial accuracy degradation. Empirically, we find that decomposing the entire FFN weight matrices with SVD often introduces excessive degradation from the original model. 
To address this, we apply low-rank SVD only to selected FFN submatrices and introduce a SVD-aware procedure to identify SVD-friendly hidden channels. Afterward, we further quantize the resulting matrices to reduce the computational cost and parameter size of the FFN layers.

Algorithm~\ref{alg:hybrid-ffn} summarizes the proposed hybrid FFN compression procedure, which consists of four steps. First, we estimate the SVD-friendliness of each FFN hidden channel by applying a temporary truncated SVD to the gate and up projections, and select the channels with the lowest reconstruction error for final SVD. Second, we move the selected channels into a contiguous block by applying the same permutation to $W_G$ and $W_U$, and the inverse permutation to $W_D$. This preserves the SwiGLU FFN output because each gate/up hidden channel remains aligned with its corresponding row in the down projection. Third, we apply SVD only to the selected gate/up blocks, while keeping the remaining channels dense. Finally, we insert an orthogonal rotation between each pair of SVD factors and apply round-to-nearest (RTN) quantization to all resulting factors and dense blocks. 

%In our implementation, we set $\gamma=50\%$ and retain $\rho_{\rm ffn}=90\%$ of the selected SVD branch parameters, and skip FFN SVD in the last five transformer layers. These empirical choices balance compression, latency reduction, and accuracy.



%Algorithm~\ref{alg:hybrid-ffn} summarizes this hybrid FFN compression procedure. The overall procedure consists of four steps. First, we estimate the SVD-friendliness of each FFN hidden channel using a temporary truncated SVD of the gate and up projections, and select the lowest-error channels for final SVD. Second, we group the selected channels into a contiguous block by applying the same permutation to $W_G$ and $W_U$, and the inverse permutation to $W_D$. This preserves the SwiGLU FFN output because each aligned gate/up hidden channel remains paired with its corresponding row in the down projection. Third, we apply SVD only to the selected gate/up blocks and keep the remaining channels dense. Finally, we insert an orthogonal rotation between each pair of SVD factors and quantize all resulting factors and dense blocks with RTN. 

% {\small
% \begin{algorithm}[t]
% \caption{SVD-aware Hybrid FFN Compression}
% \label{alg:hybrid-ffn}
% \small
% \begin{algorithmic}[1]
% \Require FFN weights $W_G,W_U \in R^{ d_{\text{in}}\times d_\text{ffn}},W_D \in R^{ d_\text{ffn}\times d_{\text{out}}}$; SVD channel ratio $\gamma$; SVD retention ratio $\rho_{\rm ffn}$
% \Ensure Quantized hybrid low-rank--dense FFN

% \State $\bar W_G,\bar W_U \leftarrow
% \mathrm{LowRank}(W_G;\rho_{\rm ffn}),\mathrm{LowRank}(W_U;\rho_{\rm ffn})$
% \Comment{temporary SVD for channel scoring}

% \For{$j=1,\ldots,d_{\rm ffn}$}
%     \State $e_j \leftarrow
%     \|W_G[:,j]-\bar W_G[:,j]\|_2^2
%     +\|W_U[:,j]-\bar W_U[:,j]\|_2^2$
%     \Comment{SVD error for each hidden channel}
% \EndFor

% \State $\mathcal{I}_S \leftarrow$ indices of the $\lfloor \gamma d_{\rm ffn}\rfloor$ smallest scores in $\{e_j\}$
% \Comment{SVD-friendly channels}
% \State $\mathcal{I}_D \leftarrow \{1,\ldots,d_{\rm ffn}\}\setminus\mathcal{I}_S$
% \Comment{other channels kept dense}

% \State $\pi \leftarrow \mathrm{Concat}(\mathcal{I}_S,\mathcal{I}_D)$
% \Comment{new channel order with SVD channels first}
% \State $P_\pi \leftarrow$ permutation matrix induced by this order
% \State $W_G',W_U',W_D' \leftarrow W_GP_\pi,\; W_UP_\pi,\; P_\pi^\top W_D$
% \Comment{preserve FFN output}

% \State $[W_{G,S}',W_{G,D}'] \leftarrow \mathrm{Split}(W_G',|\mathcal{I}_S|)$, \quad
% $[W_{U,S}',W_{U,D}'] \leftarrow \mathrm{Split}(W_U',|\mathcal{I}_S|)$
% \Comment{separate SVD and dense blocks}

% \State $(A_G,B_G),(A_U,B_U) \leftarrow
% \mathrm{LowRank}(W_{G,S}';\rho_{\rm ffn}),\;
% \mathrm{LowRank}(W_{U,S}';\rho_{\rm ffn})$
% \Comment{SVD selected blocks}

% \For{$T\in\{G,U\}$}
%     \State $R_T \leftarrow \mathrm{Rotation}(\mathrm{rank}(A_T))$
%     \Comment{orthogonal rotation: $R_T^\top R_T=I$}
%     \State $(A_T,B_T) \leftarrow (A_TR_T,R_T^\top B_T)$
%     \Comment{preserve product while smoothing factors}
%     \State $(A_{T,q},B_{T,q}) \leftarrow \mathrm{RTN}(A_T,B_T)$
% \EndFor

% \State $W_{G,D,q}',W_{U,D,q}',W_{D,q}' \leftarrow
% \mathrm{RTN}(W_{G,D}'),\mathrm{RTN}(W_{U,D}'),\mathrm{RTN}(W_D')$
% \Comment{quantize dense branch and down projection}

% \State \Return $\{A_{G,q},B_{G,q},A_{U,q},B_{U,q},
% W_{G,D,q}',W_{U,D,q}',W_{D,q}'\}$
% \end{algorithmic}
% \end{algorithm}
% }



\subsection{System Implementation}
\label{sec:mixgaup-kernel}

% \begin{wrapfigure}{r}{0.5\linewidth}
%     \vspace{-12pt}
%     \centering
%     \includegraphics[width=\linewidth]{figures/mixffn_kernel.pdf}
%     \vspace{-15pt}
%     \caption{Mix SVD-Quantization FFN kernel (MixFFN) utilize fused kernel to reduce intermediate activations load/store and kernel launch time. The detailed implmentation includes: (a) naive pytorch implementation of Matmul-SwiGLU operations. (b) fused dense branch $W_{U,D}',W_{G,D}'$ with SwiGLU. (c) fused SVD branch down projection $A_U,A_G$. (d) fused SVD branch up projection $B_U,B_G$ with SwiGLU.}
%     \label{fig:mixffn_kernel}
%     \vspace{-10pt}
% \end{wrapfigure}
\begin{wrapfigure}{r}{0.4\linewidth}
    \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{figures/kernel.pdf}
    \vspace{-15pt}
    \caption{Fused kernels for the hybrid low-rank--dense FFN. $\odot$ denotes the element-wise product in SwiGLU, and Q/D denote quantization/dequantization.}
    \label{fig:mixffn_kernel}
    \vspace{-15pt}
\end{wrapfigure}
To realize the latency benefits of LSVD’s low-rank and low-precision design in Sec.~\ref{sec:mix-quant-svd}, we implement the hybrid low-rank FFN using fused Triton kernels, as shown in Fig.~\ref{fig:mixffn_kernel}. This reduces kernel launches and intermediate memory traffic across gate/up projections, SwiGLU, and quantization/dequantization operations.

%\caption{Mix SVD-Quantization FFN kernel (MixFFN) utilize fused kernel to reduce intermediate activations load/store and kernel launch time. The detailed implmentation includes: (a) naive pytorch implementation of Matmul-SwiGLU operations. (b) fused dense branch $W_{U,D}',W_{G,D}'$ with SwiGLU. (c) fused SVD branch down projection $A_U,A_G$. (d) fused SVD branch up projection $B_U,B_G$ with SwiGLU.}

For the SVD-factorized branch in Sec.~\ref{sec:mix-quant-svd}, 
where $W_{G,S}'\approx A_{G,q}B_{G,q}$ and $W_{U,S}'\approx A_{U,q}B_{U,q}$, we first fuse the input-side projections $XA_{G,q}$ and $XA_{U,q}$ into a single kernel to generate the latent activations.
%$L_G$ and $L_U$. 
The second-stage projections with $B_{G,q}$ and $B_{U,q}$ are fused and then applied to the corresponding latent activations. For the dense branch, we likewise fuse the computation of $XW_{G,D,q}'$ and $XW_{U,D,q}'$ into one kernel.
Both branches use the same channel partition defined in Sec.~\ref{sec:mix-quant-svd}. Since the gate and up projections share aligned channel assignments, SwiGLU can be applied independently within each branch. We therefore fuse SiLU and element-wise multiplication after the projections, and then concatenate the SVD-factorized and dense outputs to obtain the final FFN activation.
For low-precision inference, we further fuse the per-token maximum reduction, quantization, and dequantization steps into the projection and nonlinear LayerNorm kernels, as shown by the Q/D nodes in Fig.~\ref{fig:mixffn_kernel}. This avoids extra passes over intermediate activations and reduces quantization-related overhead. Overall, the fused implementation preserves the original FFN computation while reducing memory movement, kernel launches, and quantization overhead. For SA layers, we extend the fused attention kernel~\cite{wang2026wsvd} to the low-precision setting to further improve inference efficiency.


\section{Evaluation}
\label{sec:eval}
% \subsection{Experimental Setup}
% \label{sec:exp-setup}
We conduct experiments on five representative vision–language models: LLaVA-v1.5 7B~\cite{liu2023visual-llava}, LLaVA-Next 7B, LLaVA-Next 13B, Qwen2-VL 7B~\cite{wang2024qwen2}, and SmolVLM 2B~\cite{marafioti2025smolvlm}. For calibration, we use 256 samples randomly drawn from the ScienceQA training split~\cite{lu2022learn_sqa}, following the procedures described in Sec.~\ref{sec:loss-aware-svd},~\ref{sec:rank-alloc} and~\ref{sec:qa-whitening}. Evaluation is conducted on three widely used benchmarks, ScienceQA-IMG~\cite{lu2022learn_sqa}, SEED-Bench-IMG~\cite{li2024seed} and MMBench~\cite{liu2024mmbench}, consistent with prior studies on VLMs such as LLaVA, using the VLMEvalKit~\cite{duan2024vlmevalkit} tool.
For comparison, LSVD is benchmarked against several baselines, including SVD-based approaches (SVD-LLM~\cite{wang2024svd}, QSVD~\cite{wang2025qsvd}, WSVD~\cite{wang2026wsvd}) and quantization-based techniques (DuQuant~\cite{lin2024duquant}, QVLM~\cite{wang2024qvlm}). For SVD-LLM, QSVD and WSVD, we follow their official implementations and apply SVD independently to the QKV projection matrices to ensure a fair comparison with LSVD, while leaving other linear layers unchanged. In addition, LSVD introduces low-rank approximation for low-precision FFN under quantized settings. For FFN optimization, we set $\gamma=50\%$ and retain $\rho_{\rm ffn}=90\%$ of the selected SVD branch parameters for Algorithm~\ref{alg:hybrid-ffn}.
We denote the parameter ratio by $\rho_1$. For rank-$r$ SVD of a per-head projection $W_h\in\mathbb{R}^{E\times H}$, where $E$ is the hidden dimension and $H$ is the head dimension, $\rho_1=(E+H)r/(EH)$, while KV-cache size is reduced by the rank ratio $r/H$.
More results are shown in the Appendix~\ref{sec:appx-results}.

To isolate the impact of SVD from quantization, we introduce \textbf{LSVD-noQ}, which applies only the loss-aware SVD and rank allocation techniques described in Sec.~\ref{sec:loss-aware-svd} and~\ref{sec:rank-alloc}. We compare it with SVD-LLM, QSVD-noQ and WSVD-noQ (unquantized version of QSVD/WSVD).
We then apply quantization-aware whitening (Sec.~\ref{sec:qa-whitening}), low-rank approximation for low-precision FFN (Sec.~\ref{sec:mix-quant-svd}) and full-model RTN quantization on top of LSVD-noQ, benchmarking against DuQuant, QVLM, QSVD and WSVD.
All experiments are conducted on NVIDIA H100 GPUs. 

\subsection{Results in FP16}
\label{sec:result-fp16}
We first evaluate the FP16 performance of LSVD-noQ under different rank budgets. To ensure fairness, we align the parameter ratio $\rho_1$ across all methods and compare their accuracy performance under the same $\rho_1$. For LSVD, $\rho_1$ is defined in Sec.~\ref{sec:eval}, while for other SVD-based baselines, $\rho_1$ is defined as the proportion of parameters relative to the original model after SVD is applied. 

\begin{table*}[t]
    \newcommand{\bc}{\cellcolor{blue!10}}
    \newcommand{\accvalours}[1]{\fontsize{9.75pt}{10pt}\selectfont \textbf{#1}}
    \centering
    \small
    \caption{Accuracy of different methods under FP16 (detailed results in Appendix~\ref{sec:appx-results-fp16}).}
    %\vspace{-5pt}
    \resizebox{\linewidth}{!}{ %
    \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    
    \multirow{2}{*}{Acc.} & \multirow{2}{*}{Method} & \multicolumn{5}{c|}{ScienceQA-IMG $\uparrow$} & \multicolumn{5}{c|}{SEED-Bench $\uparrow$} & \multirow{2}{*}{Avg. $\uparrow$ } \\
    \cmidrule{3-12}
    & & $\rho_1: 90\%$ & $\rho_1: 80\%$ & $\rho_1: 70\%$ & $\rho_1: 60\%$ & $\rho_1: 50\%$ 
    & $\rho_1: 90\%$ & $\rho_1: 80\%$ & $\rho_1: 70\%$ & $\rho_1: 60\%$ & $\rho_1: 50\%$ \\
    
    \midrule

    \multirow{5.75}{*}{\rotatebox{90}{\makecell{SmolVLM\\2B}}}

    & SVD-LLM   
        & \accval{40.06\%} & \accval{17.20\%} & \accval{3.82\%} & \accval{0.64\%} & \accval{0.69\%}
        & \accval{32.49\%} & \accval{15.89\%} & \accval{4.60\%} & \accval{3.56\%} & \accval{1.23\%}
        & \accval{12.02\%}\\
    & QSVD-noQ   
        & \accval{77.00\%} & \accval{62.77\%} & \accval{42.59\%} & \accval{9.87\%} & \accval{0.20\%}
        & \accval{64.80\%} & \accval{50.46\%} & \accval{36.24\%} & \accval{3.60\%} & \accval{2.25\%}
        & \accval{34.98\%}\\
    & WSVD-noQ   
        & \accval{76.30\%} & \accval{71.74\%} & \accval{60.93\%} & \accval{39.51\%} & \accval{27.27\%}
        & \accval{65.78\%} & \accval{63.29\%} & \accval{54.45\%} & \accval{29.22\%} & \accval{27.35\%}
        & \accval{51.58\%}\\
    %
    & \bc\textbf{LSVD-noQ} 
        & \bc\accval{\textbf{84.58\%}} & \bc\accval{\textbf{83.69\%}} & \bc\accval{\textbf{82.00\%}} & \bc\accval{\textbf{81.11\%}} & \bc\accval{\textbf{78.14\%}}
        & \bc\accval{\textbf{68.54\%}} & \bc\accval{\textbf{68.10\%}} & \bc\accval{\textbf{67.62\%}} & \bc\accval{\textbf{67.12\%}} & \bc\accval{\textbf{66.17\%}}
        & \bc\accval{\textbf{74.51\%}}\\
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 84.58\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 68.47\%}} & \textcolor{gray}{\accval{76.53\%}}\\

    % \midrule
    
    % \multirow{5.75}{*}{\rotatebox{90}{\makecell{Qwen2-VL\\7B}}}

    % & SVD-LLM   
    %     & \accval{82.80\%} & \accval{81.11\%} & \accval{80.32\%} & \accval{77.34\%} & \accval{69.31\%}
    %     & \accval{74.74\%} & \accval{74.27\%} & \accval{71.85\%} & \accval{60.83\%} & \accval{44.36\%}
    %     & \accval{71.69\%}\\
    % & QSVD-noQ   
    %     & \accval{84.09\%} & \accval{83.34\%} & \accval{82.40\%} & \accval{80.57\%} & \accval{\textbf{76.38\%}}
    %     & \accval{75.06\%} & \accval{74.97\%} & \accval{72.75\%} & \accval{70.63\%} & \accval{65.30\%}
    %     & \accval{76.55\%}\\
    % & WSVD-noQ   
    %     & \accval{82.99\%} & \accval{81.90\%} & \accval{67.38\%} & \accval{49.68\%} & \accval{15.87\%}
    %     & \accval{75.74\%} & \accval{75.27\%} & \accval{74.53\%} & \accval{72.96\%} & \accval{62.16\%}
    %     & \accval{65.85\%}\\
    % %
    % & \bc\textbf{LSVD-noQ} 
    %     & \bc\accval{\textbf{85.23\%}} & \bc\accval{\textbf{84.28\%}} & \bc\accval{\textbf{83.74\%}} & \bc\accval{\textbf{82.00\%}} & \bc\accval{75.41\%}
    %     & \bc\accval{\textbf{76.22\%}} & \bc\accval{\textbf{76.24\%}} & \bc\accval{\textbf{75.96\%}} & \bc\accval{\textbf{75.14\%}} & \bc\accval{\textbf{69.95\%}}
    %     & \bc\accval{\textbf{78.42\%}}\\
    % \cline{3-12}
    % \rule{0pt}{2.75ex}
    % & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 84.38\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 76.29\%}} & \textcolor{gray}{\accval{80.33\%}}\\

    \midrule
    
    \multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-v1.5\\7B}}}   

    & SVD-LLM  
        & \accval{65.44\%} & \accval{63.71\%} & \accval{61.92\%} & \accval{57.41\%} & \accval{55.53\%}
        & \accval{57.89\%} & \accval{57.50\%} & \accval{55.33\%} & \accval{54.64\%} & \accval{55.31\%} 
        & \accval{58.47\%}\\
    & QSVD-noQ   
        & \accval{67.72\%} & \accval{\textbf{68.22\%}} & \accval{67.08\%} & \accval{65.05\%} & \accval{62.37\%} 
        & \accval{59.84\%} & \accval{59.07\%} & \accval{59.78\%} & \accval{59.00\%} & \accval{58.23\%} 
        & \accval{62.64\%}\\
    & WSVD-noQ   
        & \accval{\textbf{68.17\%}} & \accval{67.72\%} & \accval{\textbf{67.28\%}} & \accval{65.89\%} & \accval{65.49\%}
        & \accval{60.10\%} & \accval{\textbf{60.17\%}} & \accval{59.89\%} & \accval{\textbf{60.18\%}} & \accval{60.46\%}
        & \accval{63.54\%}\\
    % & \rowcolor{blue!10}\textbf{WSVD-noQ} 
    & \bc\textbf{LSVD-noQ}
        & \bc\accval{68.12\%} & \bc\accval{68.02\%} & \bc\accval{67.03\%} & \bc\accval{\textbf{67.08\%}} & \bc\accval{\textbf{66.73\%}}
        & \bc\accval{\textbf{60.14\%}} & \bc\accval{60.00\%} & \bc\accval{\textbf{60.55\%}} & \bc\accval{59.82\%} & \bc\accval{\textbf{60.60\%}}
        & \bc\accval{\textbf{63.81\%}}\\
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 68.01\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 60.18\%}} & \textcolor{gray}{\accval{64.10\%}}  \\
    
    \midrule
    
    \multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-Next\\13B}}} %LLaVA-v1.5-13B

    & SVD-LLM    
        & \accval{72.53\%} & \accval{72.24\%} & \accval{71.74\%} & \accval{71.15\%} & \accval{70.55\%} 
        & \accval{70.76\%} & \accval{70.63\%} & \accval{70.25\%} & \accval{69.96\%} & \accval{69.58\%} 
        & \accval{70.94\%}\\
    & QSVD-noQ   
        & \accval{71.94\%} & \accval{72.14\%} & \accval{71.74\%} & \accval{72.14\%} & \accval{71.79\%} 
        & \accval{71.23\%} & \accval{71.02\%} & \accval{71.06\%} & \accval{70.92\%} & \accval{70.40\%} 
        & \accval{71.44\%}\\
    & WSVD-noQ   
        & \accval{72.88\%} & \accval{72.98\%} & \accval{\textbf{73.57\%}} & \accval{\textbf{73.48\%}} & \accval{73.28\%}
        & \accval{71.29\%} & \accval{71.17\%} & \accval{71.25\%} & \accval{70.95\%} & \accval{70.81\%}
        & \accval{72.17\%}\\
    %
    & \bc\textbf{LSVD-noQ} 
        & \bc\accval{\textbf{73.13\%}} & \bc\accval{\textbf{73.03\%}} & \bc\accval{73.38\%} & \bc\accval{73.13\%} & \bc\accval{\textbf{73.67\%}}
        & \bc\accval{\textbf{71.39\%}} & \bc\accval{\textbf{71.40\%}} & \bc\accval{\textbf{71.33\%}} & \bc\accval{\textbf{71.37\%}} & \bc\accval{\textbf{71.25\%}}
        & \bc\accval{\textbf{72.31\%}}\\
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 73.23\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 71.30\%}} & \textcolor{gray}{\accval{72.27\%}}\\
    
    
    \bottomrule
    \end{tabular}
    }
    \label{tab:svd-result}
    \vspace{-12pt}
\end{table*}
The evaluation results are summarized in Tab.~\ref{tab:svd-result}, with detailed results in Appendix~\ref{sec:appx-results-fp16}. Under the same parameter ratio $\rho_1$, LSVD-noQ surpasses SVD-LLM, QSVD-noQ, and WSVD-noQ in accuracy in most cases. On large-scale models such as LLaVA-Next 13B, LSVD-noQ incurs less than a $1\%$ accuracy drop on ScienceQA-IMG and SEED-Bench compared to the FP16 baseline. Notably, for LLaVA-Next 13B, when $\rho_1 = 50\%$, LSVD-noQ even outperforms the FP16 model on ScienceQA-IMG, exceeding the FP16 baseline by more than $0.4\%$. One possible reason is that low-rank approximation may implicitly reduce hallucinations~\citep{liu2024survey}, although this hypothesis requires further validation.
Furthermore, LSVD-noQ achieves consistently higher average accuracy across datasets and parameter ratios, with its advantage becoming more pronounced as $\rho_1$ decreases. For example, on SmolVLM, LSVD-noQ maintains over $78\%$ accuracy on ScienceQA-IMG, while other baselines fail to produce usable results under the same parameter-ratio settings.

\subsection{Results in Quantized Settings}
\label{sec:result-quant}
\begin{wraptable}{r}{0.6\linewidth}
    \vspace{-15pt}
    \centering
    \newcommand{\bc}{\cellcolor{blue!10}}
    \newcommand{\accvalours}[1]{\fontsize{9.75pt}{10pt}\selectfont \textbf{#1}}
    \small
    \caption{Accuracy evaluation of different methods under low-precision on LLaVA-v1.5 7B, Next 7B and 13B.}%(\textcolor{red}{remove the results on v1.5 13B, using wraptable})}
    \resizebox{0.98\linewidth}{!}
    {%
    \begin{tabular}{l|c|c|c|c|c|c|c}
    \toprule
    
    \multirow{2}{*}{Method} 
    & \multicolumn{3}{c|}{ScienceQA-IMG $\uparrow$} 
    & \multicolumn{3}{c|}{SEED-Bench $\uparrow$} 
    & \multirow{2}{*}{Avg. $\uparrow$} \\
    
    \cmidrule{2-7}
    
    & v1.5 7B & Next 7B & Next 13B 
    & v1.5 7B & Next 7B & Next 13B 
    & \\
    
    \midrule
    
    DuQuant   
        & \accval{57.36\%} 
        & \accval{66.34\%} 
        & \accval{70.20\%} 
        & \accval{54.11\%} 
        & \accval{63.64\%} 
        & \accval{66.15\%} 
        & \accval{62.97\%} \\
        
    QVLM 
        & \accval{55.24\%} 
        & \accval{60.60\%} 
        & \accval{65.28\%} 
        & \accval{50.13\%} 
        & \accval{50.38\%} 
        & \accval{65.39\%} 
        & \accval{57.84\%} \\
        
    QSVD 
        & \accval{65.61\%} 
        & \accval{66.10\%} 
        & \accval{70.43\%} 
        & \accval{58.49\%} 
        & \accval{65.63\%} 
        & \accval{69.21\%} 
        & \accval{65.91\%} \\
        
    WSVD 
        & \accval{64.25\%} 
        & \accval{66.94\%} 
        & \accval{\textbf{73.08\%}} 
        & \accval{60.23\%} 
        & \accval{67.49\%} 
        & \accval{70.67\%} 
        & \accval{67.11\%} \\
        
    \rowcolor{blue!10}
    \textbf{LSVD} 
        & \accval{\textbf{66.14\%}} 
        & \accval{\textbf{68.37\%}} 
        & \accval{72.11\%} 
        & \accval{\textbf{61.94\%}} 
        & \accval{\textbf{67.49\%}} 
        & \accval{\textbf{71.56\%}} 
        & \accval{\textbf{67.94\%}} \\
        
    \cline{2-8}
    
    \rule{0pt}{2.5ex}
    \textcolor{gray}{FP16} 
        & \textcolor{gray}{\accval{68.10\%}} 
        & \textcolor{gray}{\accval{69.60\%}} 
        & \textcolor{gray}{\accval{73.23\%}} 
        & \textcolor{gray}{\accval{60.18\%}} 
        & \textcolor{gray}{\accval{69.02\%}} 
        & \textcolor{gray}{\accval{71.30\%}} 
        & \textcolor{gray}{\accval{68.57\%}} \\
    
    \bottomrule
    \end{tabular}
    }
    \label{tab:svd-qat-result}
    \vspace{-10pt}
\end{wraptable}
% We present results under two weight–activation quantization configurations: W8A8 for LSVD and WSVD with rank settings $\rho_{1}=50\%$, where SVD further reduces the
% full-dimensional A8 KV cache by about $50\%$, and W8A4 for all other baselines. 
We present results under two weight--activation quantization configurations.
LSVD and WSVD use W8A8 with $\rho_{1}=50\%$: A8 halves the KV-cache storage, and SVD keeps nearly half of the K/V channels, yielding about $25\%$ of the FP16 full KV-cache size. Other baselines use W8A4 with a full-dimensional
KV cache.
This design keeps cache size and parameter size comparable across methods, 
while LSVD’s FFN SVD (Sec.~\ref{sec:mix-quant-svd}) further reduces its parameter budget, ensuring fairness in comparison. 

%For QASVD and QSVD, we adopt $\rho_1 = 100\%$ truncation to match the W8 parameter budget of other baselines. Since these methods do not employ per-head SVD, they cannot leverage latent cache representations to accelerate inference and must store the full KV cache. As a result, they are also evaluated under the A4 setting to ensure comparable cache sizes. sÍ


For activation quantization, we adopt per-token symmetric quantization. For weight quantization, we employ RTN with per-channel symmetric scaling and a learnable clipping ratio, where the clipping value is selected via linear search to minimize squared error, following QuaRot~\citep{ashkboos2024quarot}. This quantization scheme is applied to the per-head Q/K/V weight matrices and all remaining attention and feed-forward modules, ensuring that the dominant matrix multiplications in each transformer block are executed in low precision. As shown in Tab.~\ref{tab:svd-qat-result}, LSVD consistently outperforms the baselines in most cases, despite using a smaller parameter budget and the same cache size. On average across models and datasets, LSVD incurs only a modest accuracy drop of just about $0.5\%$ relative to the FP16 baseline, while reducing cache size to $25\%$ of the FP16 model. %At the same time, LSVD achieves more than 0.8\% higher average accuracy than all baselines, demonstrating that the integration of loss-aware per-head SVD, hybrid low-rank FFN, and quantization within LSVD minimizes accuracy degradation.

%not only compresses model and cache size but also helps alleviate the I/O bottleneck, thereby enabling further decoding acceleration.

% \begin{table*}[t]
%     \newcommand{\bc}{\cellcolor{blue!10}}
%     \newcommand{\accvalours}[1]{\fontsize{9.75pt}{10pt}\selectfont \textbf{#1}}
%     \centering
%     \small
%     \caption{Accuracy evaluation of different methods under low-precision on LLaVA-v1.5 7B, LLaVA-v1.5 13B, LLaVA-Next 7B and LLaVA-Next 13B. (\textcolor{red}{remove the results on v1.5 13B, using wraptable})}
%     %\vspace{-5pt}
%     \resizebox{0.9\linewidth}{!}{ %
%     \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
%     \toprule
    
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{ScienceQA-IMG $\uparrow$} & \multicolumn{4}{c|}{SEED-Bench $\uparrow$} & \multirow{2}{*}{Avg. $\uparrow$ } \\
%     \cmidrule{2-9}
%     & v1.5 7B & v1.5 13B & Next 7B & Next 13B & v1.5 7B & v1.5 13B & Next 7B & Next 13B & \\
    
%     \midrule
    
%     % QuaRot  
%     %     & \accval{63.19\%} & \accval{68.02\%} & \accval{64.53\%} & \accval{66.98\%} & \accval{58.18\%} & \accval{58.53\%} & \accval{69.09\%} & \accval{71.15\%} & \accval{64.96\%} \\
%     DuQuant   
%         & \accval{57.36\%} & \accval{67.22\%} & \accval{66.34\%} & \accval{70.20\%} & \accval{54.11\%} & \accval{61.43\%} & \accval{63.64\%} & \accval{66.15\%} & \accval{63.31\%} \\
%     QVLM 
%         & \accval{55.24\%} & \accval{66.46\%} & \accval{60.60\%} & \accval{65.28\%} & \accval{50.13\%} & \accval{59.22\%} & \accval{50.38\%} & \accval{65.39\%} & \accval{59.09\%} \\
%     QSVD 
%         & \accval{65.61\%} & \accval{70.12\%} & \accval{66.10\%} & \accval{70.43\%} & \accval{58.49\%} & \accval{\textbf{62.95\%}} & \accval{65.63\%} & \accval{69.21\%} & \accval{66.07\%} \\
%     WSVD 
%         & \accval{64.25\%} & \accval{\textbf{72.14\%}} & \accval{66.94\%} & \accval{\textbf{73.08\%}} & \accval{60.23\%} & \accval{62.01\%} & \accval{67.49\%} & \accval{70.67\%} & \accval{67.10\%} \\
%     \rowcolor{blue!10}\textbf{LSVD} 
%         & \accval{\textbf{66.14\%}} & \accval{71.43\%} & \accval{\textbf{68.37\%}} & \accval{72.11\%} & \accval{\textbf{61.94\%}} & \accval{62.78\%} & \accval{\textbf{67.49\%}} & \accval{\textbf{71.56\%}} & \accval{\textbf{67.73\%}} \\
%     \cline{2-10}
%     \rule{0pt}{2.75ex}
%     \textcolor{gray}{FP16} & 
%     \textcolor{gray}{\accval{68.10\%}} &         \textcolor{gray}{\accval{71.83\%}} & 
%     \textcolor{gray}{\accval{69.60\%}} & 
%     \textcolor{gray}{\accval{73.23\%}} & 
%     \textcolor{gray}{\accval{60.18\%}} & 
%     \textcolor{gray}{\accval{62.54\%}} & 
%     \textcolor{gray}{\accval{69.02\%}} & 
%     \textcolor{gray}{\accval{71.30\%}} & 
%     \textcolor{gray}{\accval{68.23\%}} \\
    
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tab:svd-qat-result}
%     \vspace{-10pt}
% \end{table*}   



\subsection{Ablation Studies}
\label{sec:ablation}
\paragraph{Effectiveness of Loss-aware SVD}

\begin{wraptable}{r}{0.54\textwidth}
\vspace{-10pt}
\centering
\small
\caption{Results of loss-aware SVD ablation.}
%\vspace{-5pt}
\resizebox{\linewidth}{!}{ %
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{ScienceQA-IMG $\uparrow$} & \multirow{2}{*}{Avg. $\uparrow$} \\
\cmidrule{2-6}
& v1.5 7B & Next 7B & Next 13B & Q2 7B & S 2B \\
\midrule
\textcolor{gray}{FP16}
& \textcolor{gray}{\accval{68.10\%}} 
& \textcolor{gray}{\accval{69.60\%}} 
& \textcolor{gray}{\accval{73.23\%}} 
& \textcolor{gray}{\accval{84.38\%}} 
& \textcolor{gray}{\accval{84.58\%}} 
& \textcolor{gray}{\accval{75.98\%}} \\

Vanilla
& \accval{62.87\%} 
& \accval{67.72\%} 
& \accval{71.28\%} 
& \accval{53.25\%} 
& \accval{0.00\%} 
& \accval{51.02\%} \\

LSVD
& \accval{\textbf{66.73\%}} 
& \accval{\textbf{70.80\%}} 
& \accval{\textbf{73.67\%}} 
& \accval{\textbf{75.41\%}} 
& \accval{\textbf{78.14\%}} 
& \accval{\textbf{72.95\%}} \\
\bottomrule
\end{tabular}
}
\label{tab:loss-aware-svd-ablation}
\vspace{-10pt}
\end{wraptable}

We evaluate loss-aware SVD against a vanilla SVD baseline using the same Importance Score-based rank allocation and compression ratio $\rho_1=50\%$ under FP16. The \textit{Vanilla} baseline applies SVD directly to the weights, while LSVD performs SVD in the loss-aware transformed space from Sec.~\ref{sec:loss-aware-svd}. As shown in Tab.~\ref{tab:loss-aware-svd-ablation}, LSVD consistently outperforms vanilla SVD across all models, improving average accuracy from $51.02\%$ to $72.95\%$, an $21.93\%$ gain. The improvement is especially large on Qwen2-VL 7B and SmolVLM 2B, where vanilla SVD degrades severely, while LSVD preserves much higher accuracy.

%We evaluate the effectiveness of loss-aware SVD by comparing it with a vanilla SVD baseline under the same Importance Score-based rank allocation strategy and compression ratio $\rho_1=50\%$. The \textit{Vanilla} baseline applies standard SVD to the weight matrices, while LSVD performs SVD in the loss-aware transformed space described in Sec.~\ref{sec:loss-aware-svd}. As shown in Tab.~\ref{tab:loss-aware-svd-ablation}, LSVD consistently outperforms vanilla SVD across all evaluated models. On average, LSVD improves the accuracy from 54.17\% to 72.73\%, yielding an 18.56\% gain. The improvement is especially significant on Qwen2-VL 7B and SmolVLM 2B, where vanilla SVD suffers severe degradation under aggressive compression, while LSVD preserves much higher accuracy.


% This demonstrates that loss-aware SVD provides a substantially better low-rank approximation under the same setting.  Moreover, LSVD remains only 2.56\% below the FP16 baseline on average, demonstrating that loss-aware whitening provides a substantially better low-rank approximation than standard SVD under the same compression setting.

\paragraph{Effectiveness of Loss-aware Cross-layer Rank Allocation}

\begin{wraptable}{r}{0.4\textwidth}
\vspace{-10pt}
\centering
\small
\caption{Ablation of rank allocation.}
%\vspace{-5pt}
\resizebox{\linewidth}{!}{ %
\begin{tabular}{c|c|c|c|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{ScienceQA-IMG $\uparrow$} & \multirow{2}{*}{Avg. $\uparrow$} \\
\cmidrule{2-4}
& v1.5 7B & Next 7B & Next 13B & \\
\midrule
\textcolor{gray}{FP16}
& \textcolor{gray}{\accval{68.10\%}} 
& \textcolor{gray}{\accval{69.60\%}} 
& \textcolor{gray}{\accval{73.23\%}} 
& \textcolor{gray}{\accval{70.31\%}} \\

Uniform
& \accval{58.06\%} 
& \accval{59.84\%} 
& \accval{60.63\%} 
& \accval{59.51\%} \\

SV-based
& \accval{59.05\%} 
& \accval{55.63\%} 
& \accval{68.22\%} 
& \accval{60.97\%} \\

LSVD
& \accval{\textbf{66.14\%}} 
& \accval{\textbf{68.34\%}} 
& \accval{\textbf{72.11\%}} 
& \accval{\textbf{68.86\%}} \\
\bottomrule
\end{tabular}
}
\label{tab:rank-allocation-ablation}
\vspace{-13pt}
\end{wraptable}
We evaluate the loss-aware cross-layer rank allocation in Sec.~\ref{sec:rank-alloc} by comparing it against two allocation baselines under W8A8. The \textit{Uniform} baseline keeps the same number of top-$k$ singular components in each layer, without performing cross-layer rank allocation. The \textit{SV-based} baseline follows the naive singular-value-based strategy discussed in the beginning of Sec.~\ref{sec:rank-alloc}, which ranks components globally only by their singular values. As shown in Tab.~\ref{tab:rank-allocation-ablation}, LSVD consistently outperforms both baselines across all evaluated models. On average, LSVD improves over uniform allocation by $9\%$ and over SV-based allocation by nearly $8\%$. %The gains are especially clear on LLaVA-Next 7B and LLaVA-Next 13B, where the naive allocation baselines suffer from substantial accuracy degradation. Moreover, LSVD achieves an average accuracy of 69.51\%, only 1.18\% below the FP16 baseline, demonstrating that loss-aware rank allocation effectively preserves model accuracy under the same compression setting.
Additional ablations in Appendix~\ref{sec:appx-results-ablation} further show
that QAW improves low-precision SVD, while SVD-aware permutation preserves accuracy under hybrid FFN compression.

\subsection{System Evaluation}
\label{sec:system-evaluation}
\begin{wrapfigure}{r}{0.7\linewidth}
    \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{figures/latency_lsvd.pdf}
    \vspace{-15pt}
    \caption{Latency evaluations on RTX 4090 and 5090. Dashed-line columns indicate out-of-memory cases.}
    \label{fig:eval-latency}
    %\vspace{-10pt}
\end{wrapfigure} 
We evaluate the system-level performance of LSVD under the quantized setting in Sec.~\ref{sec:result-quant}, focusing on decoding acceleration. We measure layer-wise decoding latency of LLaVA-Next 7B across attention and FFN modules using our fused kernels from Sec.~\ref{sec:mixgaup-kernel} on RTX 4090 and 5090 GPUs. We compare against Eager Attention without Flash Decoding, Palu~\citep{chang2024palu}, Flash Decoding~\citep{dao2023flashdecoding}, and WSVD~\cite{wang2026wsvd}. Flash Decoding uses SDPA, while Palu and WSVD use their official 
implementations. Eager Attention and Flash Decoding operate on the full KV cache. For low-rank methods, Palu and LSVD use $\rho_1=50\%$, reducing KV cache size by about $50\%$, 
while WSVD uses $\rho_1=60\%$ to match LSVD more closely in accuracy. Both WSVD and LSVD use INT8 W8A8 quantization, while others operate at FP16, and all measurements use batch size $32$.
As shown in Fig.~\ref{fig:eval-latency}, LSVD consistently outperforms all baselines on both GPUs, achieving on average a $4.7\times$ speedup over Flash Decoding and a $2.3\times$ speedup over WSVD. The gains come from the fused kernels in Sec.~\ref{sec:mixgaup-kernel}: the W8A8 low-rank decoding kernel reduces attention-side materialization and KV-cache memory traffic, while the hybrid FFN kernel fuses low-rank reconstruction, SwiGLU, quantization, and accumulation. By reducing memory movement and kernel launch overhead, LSVD delivers consistent decoding latency reduction across context lengths and GPUs while preserving accuracy.



%We evaluate the system-level performance of LSVD under the quantized setting as mentioned in Sec.~\ref{sec:result-quant}, with a focus on decoding-stage acceleration. Specifically, we measure the layer-wise decoding latency of LLaVA-Next 7B across the attention and feed-forward modules using our fused kernel implementation described in Sec.~\ref{sec:mixgaup-kernel} on RTX 4090 and 5090 GPUs.
%For comparison, we include Eager Attention without Flash Decoding, Palu~\citep{chang2024palu}, Flash Decoding~\citep{dao2023flashdecoding}, and WSVD~\cite{wang2026wsvd} as the baselines. 
%For Flash Decoding, we adopt scaled dot-product attention (SDPA), while Palu and WSVD are evaluated using their official repositories. Both Eager Attention and Flash Decoding operate on the full KV cache. For low-rank baselines, Palu and LSVD use $\rho_1=50\%$, compressing the KV cache by approximately $50\%$. WSVD uses $\rho_1=60\%$ so that WSVD and LSVD are compared under more comparable accuracy levels. Both WSVD and LSVD are quantized to W8A8. All measurements are conducted with a batch size of $32$.




%As shown in Fig.~\ref{fig:eval-latency}, LSVD consistently outperforms all baselines on both GPUs. On average, LSVD achieves a $4.7\times$ speedup over Flash Decoding and a $2.3\times$ speedup over WSVD. The improvement comes from two sources. First, for self-attention, our W8A8 fused low-rank decoding kernel integrates per-head low-rank Q/K/V projections with quantized execution, reducing intermediate tensor materialization, memory traffic, and kernel launch overhead. Second, for the FFN, our fused hybrid FFN kernel combines the low-rank branch, quantized branch, SwiGLU activation, and output accumulation, avoiding expensive intermediate writes across separate operators. Together, these fused kernels reduce both attention-side KV/cache-related I/O and FFN-side reconstruction overhead, leading to consistent decoding latency reduction across context lengths and GPUs. These results demonstrate that LSVD provides an effective system-level solution for practical VLM decoding acceleration while maintaining accuracy performance.
\section{Conclusion and Limitation}
\label{sec:conclusion}
LSVD provides a loss-aware low-rank compression framework for efficient VLM inference by aligning SVD with model-loss sensitivity, allocating ranks across layers and heads using calibration gradients, and extending compression to FFN layers with a hybrid SVD--quantization design. Currently, LSVD is evaluated on representative VLMs and benchmarks, and broader validation on newer architectures, longer contexts, and more aggressive low-bit settings remains future work.

{
\newpage
\small
\bibliographystyle{plainnat}
\bibliography{references}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\appendix

\section{Technical appendices and supplementary material}
% Technical appendices with additional results, figures, graphs, and proofs may be submitted with the paper submission before the full submission deadline (see above). You can upload a ZIP file for videos or code, but do not upload a separate PDF file for the appendix. There is no page limit for the technical appendices. 

% Note: Think of the appendix as ``optional reading'' for reviewers. The paper must be able to stand alone without the appendix; for example, adding critical experiments that support the main claims to an appendix is inappropriate. 
%\section{Appendix}

\subsection{K-FAC Loss Surrogate for Weight Compression}
\label{sec:appx-loss-surrogate}

\paragraph{Derivation.}
By Taylor's theorem, the loss variation induced by $\Delta W$ satisfies:
{\small
\begin{equation}
\Delta \mathcal{L}
=
\mathcal{L}(W+\Delta W)-\mathcal{L}(W)  \\
=
\langle \nabla_W\mathcal{L}(W),\Delta W\rangle
+
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
H_W
\mathrm{vec}(\Delta W)
+
O(\|\Delta W\|_F^3)
\label{eq:taylor-expansion}
\end{equation}
}
where $H_W=\nabla_W^2\mathcal{L}(W)$. For a pretrained model close to a
stationary point and a small compression perturbation, the first-order term and
higher-order remainder are negligible, giving:
{\small
\begin{equation}
\Delta \mathcal{L}
\approx
\frac{1}{2}
\mathrm{vec}(\Delta W)^{\top}
H_W
\mathrm{vec}(\Delta W)
\label{eq:hessian-loss-surrogate}
\end{equation}
}

Since directly forming the Hessian block $H_W$ is prohibitively expensive for large models, following standard natural-gradient and second-order approximations, we replace
the Hessian block with the Fisher block~\cite{amari1998natural,martens2020new},
and then use K-FAC to obtain a tractable Kronecker-factored curvature
surrogate~\cite{martens2015optimizing}. For the linear layer $y=xW$, this gives:
{\small
\begin{equation}
\begin{aligned}
H_W
&\approx F_W
=
\mathbb{E}
\!\left[
\mathrm{vec}(\nabla_W\ell)
\mathrm{vec}(\nabla_W\ell)^{\top}
\right], \qquad
\nabla_W\ell
=x^{\top}g,
\qquad
\mathrm{vec}(\nabla_W\ell)=g^{\top}\otimes x^{\top}, \\
F_W
&=
\mathbb{E}
\!\left[
(g^{\top}\otimes x^{\top})(g\otimes x)
\right] =
\mathbb{E}
\!\left[
(g^{\top}g)\otimes(x^{\top}x)
\right]
\approx
\mathbb{E}[g^{\top}g]\otimes \mathbb{E}[x^{\top}x]
=
G\otimes X
\end{aligned}
\label{eq:fisher-linear-compact}
\end{equation}
}
Here $X=\mathbb{E}[x^{\top}x]$ and $G=\mathbb{E}[g^{\top}g]$ are estimated from calibration data. Substituting $H_W\approx G\otimes X$ into Eq.~\ref{eq:hessian-loss-surrogate} yields Eq.~\ref{eq:kfac-loss-surrogate}.

\subsection{Proof of Theorem~\ref{thm:loss-aware-svd}}
\begin{proof}
Let $\Delta W=W-\widehat W_r$. From
Assumption~\ref{assm:kfac-loss-surrogate},
using $X=S_x^{\top}S_x$ and $G=S_gS_g^{\top}$, together with the Kronecker-product identities $(A\otimes B)(C\otimes D)=(AC)\otimes(BD)$ and $\mathrm{vec}(ABC)=(C^{\top}\otimes A)\mathrm{vec}(B)$, we obtain:
{\small
\begin{equation}
\begin{aligned}
\Delta\mathcal{L}
&\approx
\frac{1}{2}\mathrm{vec}(\Delta W)^{\top}
(G\otimes X)
\mathrm{vec}(\Delta W) 
=
\frac{1}{2}\mathrm{vec}(\Delta W)^{\top}
(S_gS_g^{\top}\otimes S_x^{\top}S_x)
\mathrm{vec}(\Delta W) \\
&=
\frac{1}{2}\mathrm{vec}(\Delta W)^{\top}
(S_g\otimes S_x^{\top})(S_g^{\top}\otimes S_x)
\mathrm{vec}(\Delta W) 
=
\frac{1}{2}\left\|
(S_g^{\top}\otimes S_x)\mathrm{vec}(\Delta W)
\right\|_2^2 \\
&=
\frac{1}{2}\left\|
\mathrm{vec}(S_x\Delta W S_g)
\right\|_2^2
=
\frac{1}{2}\left\|
S_x\Delta W S_g
\right\|_F^2
\label{eq:kfac-to-weighted-frobenius}
\end{aligned}
\end{equation}
}
Therefore, minimizing the estimated loss increase in Assumption~\ref{assm:kfac-loss-surrogate} over rank-$r$ approximations is equivalent to:
{\small
\begin{equation}
\min_{\operatorname{rank}(\widehat W_r)\le r}
\left\|S_x(W-\widehat W_r)S_g\right\|_F^2
\label{eq:loss-aware-svd-objective}
\end{equation}
}
Define the curvature-weighted weight and rank-$r$ approximation as $\widetilde W=S_xWS_g$ and $\widetilde W_r=S_x\widehat W_rS_g$. Since $S_x$ and $S_g$ are nonsingular, left and right multiplication by them is 
% one-to-one and 
rank-preserving. Thus Eq.~\ref{eq:loss-aware-svd-objective} reduces to the standard Frobenius-norm rank-$r$ approximation problem:
{\small
\begin{equation}
\min_{\operatorname{rank}(\widetilde W_r)\le r}
\left\|\widetilde W-\widetilde W_r\right\|_F^2
\label{eq:standard-rank-r-proof}
\end{equation}
}
By the Eckart--Young--Mirsky theorem~\cite{eckart1936approximation,mirsky1960symmetric},
the optimal solution is the truncated SVD
$\widetilde W_r^{\star}=U_r\Sigma_rV_r^{\top}$. Mapping it back to the original weight space gives:
{\small
\begin{equation}
\widehat W_r^{\star}
=
S_x^{-1}\widetilde W_r^{\star}S_g^{-1}
=
S_x^{-1}U_r\Sigma_rV_r^{\top}S_g^{-1}
\end{equation}
}
Moreover, the optimal residual in the transformed space is
$\|\widetilde W-\widetilde W_r^{\star}\|_F^2=\sum_{i=r+1}^{q}\sigma_i^2$.
Substituting this residual into Eq.~\ref{eq:kfac-to-weighted-frobenius} gives:
$\Delta\mathcal{L}_r\approx\frac{1}{2}\sum_{i=r+1}^{q}\sigma_i^2$.
This proves Theorem~\ref{thm:loss-aware-svd}.
\end{proof}

\subsection{K-FAC Approximation Error Analysis}
\label{sec:appx-scale-diag}


We analyze why the local loss estimate
$\frac{1}{2}\sigma_{\ell,i}^{2}$ obtained in the loss-aware transformed space
is useful within one layer or head, but may not be directly comparable across
different layers or heads. Let $F_\ell$ denote the empirical Fisher matrix of
layer $\ell$, and let
\[
K_\ell = G_\ell \otimes X_\ell
\]
be the Kronecker-factored approximation used in
Assumption~\ref{assm:kfac-loss-surrogate}. We write the difference between the
empirical Fisher and this K-FAC approximation as:
\[
F_\ell = K_\ell + R_\ell,
\qquad
R_\ell \triangleq F_\ell - K_\ell
\]
Here, $R_\ell$ contains the curvature information that is not captured by the
Kronecker factorization.

For the $i$-th loss-aware singular value of layer $\ell$, $\sigma_{\ell,i}$, let:
\[
W_{\ell,i}^{\mathrm{svd}}
=
S_{x,\ell}^{-1}
\sigma_{\ell,i}u_{\ell,i}v_{\ell,i}^{\top}
S_{g,\ell}^{-1}
\]
denote the corresponding rank-one component mapped back to the original
weight space. Dropping this component induces the weight perturbation:
\[
\Delta W_{\ell,i}^{\mathrm{drop}}
=
-W_{\ell,i}^{\mathrm{svd}},
\qquad
z_{\ell,i}
=
\operatorname{vec}(\Delta W_{\ell,i}^{\mathrm{drop}}).
\]
Here, $W_{\ell,i}^{\mathrm{svd}}$ denotes the component itself, while
$\Delta W_{\ell,i}^{\mathrm{drop}}$ denotes the perturbation caused by
removing it. The minus sign does not affect the following quadratic loss
estimate.

For this discarded loss-aware singular component 
$z_{\ell,i}=\operatorname{vec}(\Delta W_{\ell,i}^{\mathrm{drop}})$, the
empirical-Fisher second-order loss estimate can be decomposed as:
{\small
\begin{equation}
\begin{aligned}
\Delta\mathcal{L}^{F}_{\ell,i}
&\approx
\frac{1}{2} z_{\ell,i}^{\top}F_\ell z_{\ell,i}  \\
&=
\frac{1}{2} z_{\ell,i}^{\top}K_\ell z_{\ell,i}
+
\frac{1}{2} z_{\ell,i}^{\top}(F_\ell-K_\ell)z_{\ell,i} \\
&\triangleq
T^{\mathrm{KFAC}}_{\ell,i}
+
T^{\mathrm{res}}_{\ell,i}
\end{aligned}
\label{eq:fisher-kfac-decomp}
\end{equation}
}
By Theorem~\ref{thm:loss-aware-svd}, the K-FAC-based term is:
\[
T^{\mathrm{KFAC}}_{\ell,i}
=
\frac{1}{2}
\|S_{x,\ell}\Delta W_{\ell,i}^{\mathrm{drop}}S_{g,\ell}\|_F^2
=
\frac{1}{2}\sigma_{\ell,i}^{2}
\]
Thus, $\frac{1}{2}\sigma_{\ell,i}^{2}$ is the loss increase predicted by the
K-FAC surrogate when the $i$-th loss-aware singular component is removed. This
estimate is suitable for comparing components within the same layer or head,
because all candidates are evaluated under the same local approximation.
However, when components from different layers or heads are ranked together,
the K-FAC surrogate in each layer or head may over- or under-estimate the
empirical-Fisher loss by a different amount.

To make this difference explicit, 
we compare the empirical-Fisher and K-FAC approximation using the trace ratio:
%we compare the empirical-Fisher
%curvature with the K-FAC curvature using the trace ratio:
{\small
\begin{equation}
\eta_\ell
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(K_\ell)}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(G_\ell\otimes X_\ell)}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(G_\ell)\operatorname{Tr}(X_\ell)}
\label{eq:eta-diagnostic}
\end{equation}
}
The trace measures the total curvature mass of a positive semi-definite matrix.
Therefore, $\eta_\ell$ indicates whether the K-FAC surrogate tends to under- or
over-estimate the empirical-Fisher loss scale on average. Specifically,
$\eta_\ell>1$ means that K-FAC underestimates the total empirical-Fisher
curvature of layer $\ell$, while $\eta_\ell<1$ means that it overestimates it.

\paragraph{Derivation.}
To interpret this trace ratio, consider an isotropic perturbation $z=au$ in the
vectorized weight space of layer $\ell$, where $a>0$ and
$\mathbb{E}_{u}[uu^\top]=I/d_\ell$. For any symmetric curvature matrix $C$, the
quadratic loss surrogate along $z=au$ satisfies:
{\small
\begin{equation}
\mathbb{E}_{u}\!\left[\frac{1}{2}z^\top C z\right]
=
\frac{a^2}{2}\mathbb{E}_{u}[u^\top C u]
\label{eq:eta-indicator-proof-step1}
\end{equation}
}
Using $u^\top C u=\operatorname{Tr}(Cuu^\top)$ and
$\mathbb{E}_{u}[uu^\top]=I/d_\ell$, we have:
{\small
\begin{equation}
\mathbb{E}_{u}[u^\top C u]
=
\operatorname{Tr}\!\left(C\mathbb{E}_{u}[uu^\top]\right)
=
\frac{1}{d_\ell}\operatorname{Tr}(C)
\label{eq:eta-indicator-proof-step2}
\end{equation}
}
Therefore,
\[
\mathbb{E}_{u}\!\left[\frac{1}{2}z^\top C z\right]
=
\frac{a^2}{2d_\ell}\operatorname{Tr}(C)
\]
Applying this result to $C=F_\ell$ and $C=K_\ell$ cancels the common factor
$a^2/(2d_\ell)$ and gives:
{\small
\begin{equation}
\frac{
\mathbb{E}_{u}\!\left[\frac{1}{2}z^\top F_\ell z\right]
}{
\mathbb{E}_{u}\!\left[\frac{1}{2}z^\top K_\ell z\right]
}
=
\frac{\operatorname{Tr}(F_\ell)}
{\operatorname{Tr}(K_\ell)}
=
\eta_\ell
\label{eq:eta-scale-ratio}
\end{equation}
}
Similarly, applying the same result to $C=F_\ell-K_\ell$ gives the
direction-averaged relative error of the K-FAC curvature:
{\small
\begin{equation}
\frac{
\mathbb{E}_{u}\!\left[\frac{1}{2}z^\top (F_\ell-K_\ell) z\right]
}{
\mathbb{E}_{u}\!\left[\frac{1}{2}z^\top K_\ell z\right]
}
=
\eta_\ell - 1
\label{eq:eta-residual-ratio}
\end{equation}
}
Finally, since $K_\ell=G_\ell\otimes X_\ell$, the Kronecker trace identity gives:
\[
\operatorname{Tr}(K_\ell)
=
\operatorname{Tr}(G_\ell\otimes X_\ell)
=
\operatorname{Tr}(G_\ell)\operatorname{Tr}(X_\ell)
\]
which yields Eq.~\ref{eq:eta-diagnostic}.

This derivation shows that $\eta_\ell$ is a simple indicator of how the
K-FAC-based loss estimate compares with the empirical-Fisher loss estimate on
average. It is not a per-component correction, because the exact residual term
$T^{\mathrm{res}}_{\ell,i}$ depends on the direction of the discarded
component. However, large variation in $\eta_\ell$ across layers or heads means
that $\frac{1}{2}\sigma_{\ell,i}^{2}$ may not put all components on the same
loss scale. Therefore, directly sorting components from different layers or
heads by $\sigma_{\ell,i}^{2}$ can lead to inaccurate global rank allocation.

The trace-ratio indicator is also easy to compute in practice. Since the trace
only depends on diagonal entries, we do not need to materialize the full
empirical Fisher. Instead, we only need its diagonal entries, which can be
estimated from calibration gradients. For each calibration sample $n$, we run
a forward and backward pass, collect the per-sample gradient
$\nabla_{W_\ell}\ell_n$, square it elementwise, and accumulate it over the
calibration set:
\[
\mathbf f_{\ell}^{\mathrm{diag}}
\approx
\frac{1}{N}
\sum_{n=1}^{N}
\operatorname{vec}(\nabla_{W_\ell}\ell_n)
\odot
\operatorname{vec}(\nabla_{W_\ell}\ell_n)
\]
where $\mathbf f_{\ell}^{\mathrm{diag}}$ is a vector that estimates the
diagonal entries of the empirical Fisher, and $\odot$ denotes elementwise
multiplication. Summing its entries gives the empirical-Fisher trace:
{\small
\begin{equation}
\operatorname{Tr}(F_\ell)
=
\sum_j [F_\ell]_{j,j}
\approx
\sum_j [\mathbf f_{\ell}^{\mathrm{diag}}]_j
=
\frac{1}{N}
\sum_{n=1}^{N}
\left\|
\nabla_{W_\ell}\ell_n
\right\|_F^2 .
\label{eq:diag-fisher-trace}
\end{equation}
}
Thus, the practical computation only requires two trace values:
$\operatorname{Tr}(F_\ell)$ and $\operatorname{Tr}(K_\ell)$. The
empirical-Fisher trace $\operatorname{Tr}(F_\ell)$ is estimated by accumulating
squared per-sample calibration gradients, while the K-FAC trace
$\operatorname{Tr}(K_\ell)$ is computed directly from the Kronecker factors:
\[
\operatorname{Tr}(K_\ell)
=
\operatorname{Tr}(G_\ell\otimes X_\ell)
=
\operatorname{Tr}(G_\ell)\operatorname{Tr}(X_\ell)
\]
We estimate both quantities on the same calibration set used for loss-aware SVD
and rank allocation. This analysis supports the observation in
Sec.~\ref{sec:rank-alloc}: the local loss estimate
$\frac{1}{2}\sigma_{\ell,i}^{2}$ is useful for deciding which components to
truncate within a layer or head, but it is not always reliable for ranking
components globally. This motivates the empirical-Fisher importance score
derived in Appendix~\ref{sec:appx-importance-score}, which keeps the
loss-aware SVD basis while calibrating each singular component on a shared
empirical loss scale.



\subsection{Loss-Aware Rank Allocation}
\label{sec:appx-importance-score}

We provide the derivation of the calibration-gradient-based importance score
used for global rank allocation. For a target layer $\ell$, let the
loss-aware SVD of the curvature-weighted weight be
$\widetilde W_\ell=S_{x,\ell}W_\ell S_{g,\ell}
=U_\ell \Sigma_\ell V_\ell^\top$, where
$\Sigma_\ell=\operatorname{diag}(\sigma_{\ell,1},\ldots,\sigma_{\ell,q_\ell})$.
The rank-one component corresponding to the $i$-th singular value $\sigma_{\ell,i}$ in the original weight space is:
\[
W_{\ell,i}^{\mathrm{svd}}
=
S_{x,\ell}^{-1}
\sigma_{\ell,i}u_{\ell,i}v_{\ell,i}^{\top}
S_{g,\ell}^{-1}
\]
Under the local K-FAC surrogate, discarding this component gives the
loss estimate $\frac{1}{2}\sigma_{\ell,i}^{2}$. As discussed in
Sec.~\ref{sec:rank-alloc}, this quantity is meaningful for
local truncation within the same layer or head, but its scale may not be
directly comparable across different layers or heads.

To obtain a shared empirical scale for global rank allocation, we estimate the
loss increase of removing each loss-aware singular component under the empirical
Fisher. Recall that LSVD performs SVD on the curvature-whitened weight
$\widetilde W_\ell=S_{x,\ell}W_\ell S_{g,\ell}
=U_\ell\Sigma_\ell V_\ell^\top$. We introduce a binary mask $m_{\ell,i}$ for
each singular component in this whitened space:
\[
\widetilde W_\ell(m)
=
\sum_{i=1}^{q_\ell}
m_{\ell,i}\sigma_{\ell,i}u_{\ell,i}v_{\ell,i}^{\top}
\]
Mapping it back to the original weight space gives:
\[
\widehat W_\ell(m)
=
S_{x,\ell}^{-1}\widetilde W_\ell(m)S_{g,\ell}^{-1}
=
\sum_{i=1}^{q_\ell}
m_{\ell,i}
S_{x,\ell}^{-1}
\sigma_{\ell,i}u_{\ell,i}v_{\ell,i}^{\top}
S_{g,\ell}^{-1}
\]
Therefore, removing the $i$-th loss-aware singular component corresponds to the
weight perturbation:
\[
\Delta W_{\ell,i}^{\mathrm{drop}}
=
-W_{\ell,i}^{\mathrm{svd}}
=
-
S_{x,\ell}^{-1}
\sigma_{\ell,i}u_{\ell,i}v_{\ell,i}^{\top}
S_{g,\ell}^{-1}
\]

Using the second-order loss approximation with the empirical Fisher
$F_\ell=\mathbb{E}[\mathrm{vec}(\nabla_{W_\ell}\ell)
\mathrm{vec}(\nabla_{W_\ell}\ell)^\top]$, the loss increase caused by this perturbation is:
\[
\Delta \mathcal{L}_{\ell,i}
\approx
\frac{1}{2}
\mathrm{vec}(\Delta W_{\ell,i}^{\mathrm{drop}})^\top
F_\ell
\mathrm{vec}(\Delta W_{\ell,i}^{\mathrm{drop}})
\]
Substituting the empirical Fisher form gives:
\[
\Delta \mathcal{L}_{\ell,i}
\approx
\frac{1}{2}
\mathbb{E}_{n}
\left[
\left\langle
\nabla_{W_\ell}\ell_n,
\Delta W_{\ell,i}^{\mathrm{drop}}
\right\rangle^2
\right]
\]
where $\ell_n$ is the calibration loss of the $n$-th sample. Since the sign of
$\Delta W_{\ell,i}^{\mathrm{drop}}$ is removed by the square, we obtain:
\[
\Delta \mathcal{L}_{\ell,i}
\approx
\frac{1}{2}
\sigma_{\ell,i}^{2}
\mathbb{E}_{n}
\left[
\left(
u_{\ell,i}^{\top}
S_{x,\ell}^{-T}
\nabla_{W_\ell}\ell_n
S_{g,\ell}^{-T}
v_{\ell,i}
\right)^2
\right]
\]
Equivalently, by defining the whitened-space gradient
\[
\nabla_{\widetilde W_\ell}\ell_n
=
S_{x,\ell}^{-T}
\nabla_{W_\ell}\ell_n
S_{g,\ell}^{-T}
\]
the score becomes
\[
s_{\ell,i}
=
\frac{1}{2}
\sigma_{\ell,i}^{2}
\mathbb{E}_{n}
\left[
\left(
u_{\ell,i}^{\top}
\nabla_{\widetilde W_\ell}\ell_n
v_{\ell,i}
\right)^2
\right]
\]
In practice, we estimate the expectation with the calibration set:
\[
s_{\ell,i}
=
\frac{1}{2N}
\sigma_{\ell,i}^{2}
\sum_{n=1}^{N}
\left(
u_{\ell,i}^{\top}
\nabla_{\widetilde W_\ell}\ell_n
v_{\ell,i}
\right)^2
\]
This score measures the empirical-Fisher loss increase of removing each
loss-aware singular component. The constant factor $\frac{1}{2}$ is shared by
all components and does not affect the global ranking, so we omit it and obtain
the importance score used in the main text:
\[
I_{\ell,i}
=
\frac{1}{N}
\sigma_{\ell,i}^{2}
\sum_{n=1}^{N}
\left(
u_{\ell,i}^{\top}
\nabla_{\widetilde W_\ell}\ell_n
v_{\ell,i}
\right)^2
\]
Compared with directly ranking by the K-FAC-predicted local value
$\sigma_{\ell,i}^2$, this score keeps the loss-aware SVD basis induced by
$S_{x,\ell}$ and $S_{g,\ell}$ while calibrating each component on a shared
empirical loss scale across layers and heads.

\subsection{Results}
\label{sec:appx-results}

\subsubsection{More Results in FP16}
\label{sec:appx-results-fp16}

\begin{table*}[h]
    \newcommand{\bc}{\cellcolor{blue!10}}
    \newcommand{\accvalours}[1]{\fontsize{9.75pt}{10pt}\selectfont \textbf{#1}}
    \centering
    \small
    \caption{Accuracy evaluation of different methods under FP16.}
    %\vspace{-5pt}
    \resizebox{\linewidth}{!}{ %
    \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    
    \multirow{2}{*}{Acc.} & \multirow{2}{*}{Method} & \multicolumn{5}{c|}{ScienceQA-IMG $\uparrow$} & \multicolumn{5}{c|}{SEED-Bench $\uparrow$} & \multirow{2}{*}{Avg. $\uparrow$ } \\
    \cmidrule{3-12}
    & & $\rho_1: 90\%$ & $\rho_1: 80\%$ & $\rho_1: 70\%$ & $\rho_1: 60\%$ & $\rho_1: 50\%$ 
    & $\rho_1: 90\%$ & $\rho_1: 80\%$ & $\rho_1: 70\%$ & $\rho_1: 60\%$ & $\rho_1: 50\%$ \\
    
    \midrule

    \multirow{5.75}{*}{\rotatebox{90}{\makecell{SmolVLM\\2B}}}

    & SVD-LLM   
        & \accval{40.06\%} & \accval{17.20\%} & \accval{3.82\%} & \accval{0.64\%} & \accval{0.69\%}
        & \accval{32.49\%} & \accval{15.89\%} & \accval{4.60\%} & \accval{3.56\%} & \accval{1.23\%}
        & \accval{12.02\%}\\
    & QSVD-noQ   
        & \accval{77.00\%} & \accval{62.77\%} & \accval{42.59\%} & \accval{9.87\%} & \accval{0.20\%}
        & \accval{64.80\%} & \accval{50.46\%} & \accval{36.24\%} & \accval{3.60\%} & \accval{2.25\%}
        & \accval{34.98\%}\\
    & WSVD-noQ   
        & \accval{76.30\%} & \accval{71.74\%} & \accval{60.93\%} & \accval{39.51\%} & \accval{27.27\%}
        & \accval{65.78\%} & \accval{63.29\%} & \accval{54.45\%} & \accval{29.22\%} & \accval{27.35\%}
        & \accval{51.58\%}\\
    %
    & \bc\textbf{LSVD-noQ} 
        & \bc\accval{\textbf{84.58\%}} & \bc\accval{\textbf{83.69\%}} & \bc\accval{\textbf{82.00\%}} & \bc\accval{\textbf{81.11\%}} & \bc\accval{\textbf{78.14\%}}
        & \bc\accval{\textbf{68.54\%}} & \bc\accval{\textbf{68.10\%}} & \bc\accval{\textbf{67.62\%}} & \bc\accval{\textbf{67.12\%}} & \bc\accval{\textbf{66.17\%}}
        & \bc\accval{\textbf{74.51\%}}\\
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 84.58\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 68.47\%}} & \textcolor{gray}{\accval{76.53\%}}\\

    \midrule
    
    \multirow{5.75}{*}{\rotatebox{90}{\makecell{Qwen2-VL\\7B}}}

    & SVD-LLM   
        & \accval{82.80\%} & \accval{81.11\%} & \accval{80.32\%} & \accval{77.34\%} & \accval{69.31\%}
        & \accval{74.74\%} & \accval{74.27\%} & \accval{71.85\%} & \accval{60.83\%} & \accval{44.36\%}
        & \accval{71.69\%}\\
    & QSVD-noQ   
        & \accval{84.09\%} & \accval{83.34\%} & \accval{82.40\%} & \accval{80.57\%} & \accval{\textbf{76.38\%}}
        & \accval{75.06\%} & \accval{74.97\%} & \accval{72.75\%} & \accval{70.63\%} & \accval{65.30\%}
        & \accval{76.55\%}\\
    & WSVD-noQ   
        & \accval{82.99\%} & \accval{81.90\%} & \accval{67.38\%} & \accval{49.68\%} & \accval{15.87\%}
        & \accval{75.74\%} & \accval{75.27\%} & \accval{74.53\%} & \accval{72.96\%} & \accval{62.16\%}
        & \accval{65.85\%}\\
    %
    & \bc\textbf{LSVD-noQ} 
        & \bc\accval{\textbf{85.23\%}} & \bc\accval{\textbf{84.28\%}} & \bc\accval{\textbf{83.74\%}} & \bc\accval{\textbf{82.00\%}} & \bc\accval{75.41\%}
        & \bc\accval{\textbf{76.22\%}} & \bc\accval{\textbf{76.24\%}} & \bc\accval{\textbf{75.96\%}} & \bc\accval{\textbf{75.14\%}} & \bc\accval{\textbf{69.95\%}}
        & \bc\accval{\textbf{78.42\%}}\\
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 84.38\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 76.29\%}} & \textcolor{gray}{\accval{80.33\%}}\\

    \midrule
    
    \multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-v1.5\\7B}}}   

    & SVD-LLM  
        & \accval{65.44\%} & \accval{63.71\%} & \accval{61.92\%} & \accval{57.41\%} & \accval{55.53\%}
        & \accval{57.89\%} & \accval{57.50\%} & \accval{55.33\%} & \accval{54.64\%} & \accval{55.31\%} 
        & \accval{58.47\%}\\
    & QSVD-noQ   
        & \accval{67.72\%} & \accval{\textbf{68.22\%}} & \accval{67.08\%} & \accval{65.05\%} & \accval{62.37\%} 
        & \accval{59.84\%} & \accval{59.07\%} & \accval{59.78\%} & \accval{59.00\%} & \accval{58.23\%} 
        & \accval{62.64\%}\\
    & WSVD-noQ   
        & \accval{\textbf{68.17\%}} & \accval{67.72\%} & \accval{\textbf{67.28\%}} & \accval{65.89\%} & \accval{65.49\%}
        & \accval{60.10\%} & \accval{\textbf{60.17\%}} & \accval{59.89\%} & \accval{\textbf{60.18\%}} & \accval{60.46\%}
        & \accval{63.54\%}\\
    % & \rowcolor{blue!10}\textbf{WSVD-noQ} 
    & \bc\textbf{LSVD-noQ}
        & \bc\accval{68.12\%} & \bc\accval{68.02\%} & \bc\accval{67.03\%} & \bc\accval{\textbf{67.08\%}} & \bc\accval{\textbf{66.73\%}}
        & \bc\accval{\textbf{60.14\%}} & \bc\accval{60.00\%} & \bc\accval{\textbf{60.55\%}} & \bc\accval{59.82\%} & \bc\accval{\textbf{60.60\%}}
        & \bc\accval{\textbf{63.81\%}}\\
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 68.01\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 60.18\%}} & \textcolor{gray}{\accval{64.10\%}}  \\

    \midrule

    % \multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-v1.5\\13B}}}
    
    % & SVD-LLM
    % & \accval{71.05\%} & \accval{70.85\%} & \accval{70.30\%} & \accval{70.35\%} & \accval{70.30\%}
    % & \accval{62.28\%} & \accval{62.34\%} & \accval{62.25\%} & \accval{62.08\%} & \accval{\textbf{63.01\%}}
    % & \accval{66.48\%}\\
    
    % & QSVD-noQ
    % & \accval{71.89\%} & \accval{\textbf{71.99\%}} & \accval{71.49\%} & \accval{71.54\%} & \accval{71.39\%}
    % & \accval{\textbf{62.61\%}} & \accval{62.64\%} & \accval{\textbf{62.82\%}} & \accval{\textbf{62.63\%}} & \accval{62.52\%}
    % & \accval{67.15\%}\\
    
    % & WSVD-noQ
    % & \accval{\textbf{71.99\%}} & \accval{71.84\%} & \accval{\textbf{72.53\%}} & \accval{71.59\%} & \accval{71.44\%}
    % & \accval{62.52\%} & \accval{\textbf{62.68\%}} & \accval{62.38\%} & \accval{62.37\%} & \accval{62.37\%}
    % & \accval{67.17\%}\\
    
    % & \bc\textbf{LSVD-noQ}
    % & \bc\accval{71.89\%} & \bc\accval{71.69\%} & \bc\accval{72.24\%} & \bc\accval{\textbf{72.53\%}} & \bc\accval{\textbf{71.64\%}}
    % & \bc\accval{62.49\%} & \bc\accval{62.50\%} & \bc\accval{62.56\%} & \bc\accval{62.54\%} & \bc\accval{62.34\%}
    % & \bc\accval{\textbf{67.24\%}}\\
    
    % \cline{3-12}
    % \rule{0pt}{2.75ex}
    % & \textcolor{gray}{FP16}
    % & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 71.83\%}}
    % & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 62.53\%}}
    % & \textcolor{gray}{\accval{67.18\%}}\\
    
    % \midrule
    
    \multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-Next\\7B}}}
    
    & SVD-LLM
    & \accval{68.27\%} & \accval{67.92\%} & \accval{66.58\%} & \accval{66.39\%} & \accval{65.54\%}
    & \accval{68.50\%} & \accval{68.31\%} & \accval{67.65\%} & \accval{67.45\%} & \accval{66.28\%}
    & \accval{67.29\%}\\
    
    & QSVD-noQ
    & \accval{\textbf{70.10\%}} & \accval{69.16\%} & \accval{69.01\%} & \accval{68.27\%} & \accval{66.19\%}
    & \accval{68.86\%} & \accval{68.95\%} & \accval{68.44\%} & \accval{67.98\%} & \accval{67.27\%}
    & \accval{68.42\%}\\
    
    & WSVD-noQ
    & \accval{69.81\%} & \accval{69.56\%} & \accval{69.36\%} & \accval{68.22\%} & \accval{67.87\%}
    & \accval{69.18\%} & \accval{69.27\%} & \accval{\textbf{69.15\%}} & \accval{69.16\%} & \accval{68.59\%}
    & \accval{69.02\%}\\
    
    & \bc\textbf{LSVD-noQ}
    & \bc\accval{69.51\%} & \bc\accval{\textbf{69.81\%}} & \bc\accval{\textbf{69.86\%}} & \bc\accval{\textbf{69.86\%}} & \bc\accval{\textbf{70.80\%}}
    & \bc\accval{\textbf{69.25\%}} & \bc\accval{\textbf{69.29\%}} & \bc\accval{69.13\%} & \bc\accval{\textbf{69.34\%}} & \bc\accval{\textbf{68.77\%}}
    & \bc\accval{\textbf{69.45\%}}\\
    
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16}
    & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 69.60\%}}
    & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 69.02\%}}
    & \textcolor{gray}{\accval{69.31\%}} \\
    \midrule
    
    \multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-Next\\13B}}} %LLaVA-v1.5-13B

    & SVD-LLM    
        & \accval{72.53\%} & \accval{72.24\%} & \accval{71.74\%} & \accval{71.15\%} & \accval{70.55\%} 
        & \accval{70.76\%} & \accval{70.63\%} & \accval{70.25\%} & \accval{69.96\%} & \accval{69.58\%} 
        & \accval{70.94\%}\\
    & QSVD-noQ   
        & \accval{71.94\%} & \accval{72.14\%} & \accval{71.74\%} & \accval{72.14\%} & \accval{71.79\%} 
        & \accval{71.23\%} & \accval{71.02\%} & \accval{71.06\%} & \accval{70.92\%} & \accval{70.40\%} 
        & \accval{71.44\%}\\
    & WSVD-noQ   
        & \accval{72.88\%} & \accval{72.98\%} & \accval{\textbf{73.57\%}} & \accval{\textbf{73.48\%}} & \accval{73.28\%}
        & \accval{71.29\%} & \accval{71.17\%} & \accval{71.25\%} & \accval{70.95\%} & \accval{70.81\%}
        & \accval{72.17\%}\\
    %
    & \bc\textbf{LSVD-noQ} 
        & \bc\accval{\textbf{73.13\%}} & \bc\accval{\textbf{73.03\%}} & \bc\accval{73.38\%} & \bc\accval{73.13\%} & \bc\accval{\textbf{73.67\%}}
        & \bc\accval{\textbf{71.39\%}} & \bc\accval{\textbf{71.40\%}} & \bc\accval{\textbf{71.33\%}} & \bc\accval{\textbf{71.37\%}} & \bc\accval{\textbf{71.25\%}}
        & \bc\accval{\textbf{72.31\%}}\\
    \cline{3-12}
    \rule{0pt}{2.75ex}
    & \textcolor{gray}{FP16} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 73.23\%}} & \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 71.30\%}} & \textcolor{gray}{\accval{72.27\%}}\\
    
    
    \bottomrule
    \end{tabular}
    }
    \label{tab:appx-svd-result}
    %\vspace{-10pt}
\end{table*}

The FP16 results in Tab.~\ref{tab:appx-svd-result} further support the robustness of LSVD under a wide range
of low-rank compression ratios. Compared with SVD-LLM, QSVD-noQ, and WSVD-noQ,
LSVD-noQ consistently preserves higher accuracy as the parameter-size ratio
$\rho_1$ decreases. The advantage is especially clear under aggressive
compression. For example, on SmolVLM-2B, several baselines degrade sharply at
$\rho_1=50\%$, while LSVD-noQ still maintains strong performance on both
ScienceQA-IMG and SEED-Bench. Similar trends are observed on Qwen2-VL,
LLaVA-v1.5, and LLaVA-Next models, showing that the proposed loss-aware
decomposition is not specific to a single architecture.

\begin{table}[h]
%\vspace{-10pt}
\newcommand{\bc}{\cellcolor{blue!10}}
    \newcommand{\accvalours}[1]{\fontsize{9.75pt}{10pt}\selectfont \textbf{#1}}
\centering
\small
\caption{Accuracy evaluation of different methods on MMBench under FP16 low-rank compression.}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{c|c|ccccc|c}
\toprule
\multirow{2}{*}{Acc.} & \multirow{2}{*}{Method}
& \multicolumn{5}{c|}{MMBench EN V1.1 $\uparrow$}
& \multirow{2}{*}{Avg. $\uparrow$} \\
\cmidrule(lr){3-7}
& & $\rho_1$: 90\% & $\rho_1$: 80\% & $\rho_1$: 70\% & $\rho_1$: 60\% & $\rho_1$: 50\% & \\
\midrule

\multirow{5.75}{*}{\rotatebox{90}{\makecell{SmolVLM\\2B}}}
& SVD-LLM
& \accval{44.31\%} & \accval{33.04\%} & \accval{15.74\%} & \accval{0.73\%} & \accval{0.31\%}
& \accval{18.83\%}\\
& QSVD-noQ
& \accval{58.39\%} & \accval{52.62\%} & \accval{35.79\%} & \accval{3.38\%} & \accval{0.88\%}
& \accval{30.21\%}\\
& WSVD-noQ
& \accval{59.06\%} & \accval{55.90\%} & \accval{51.22\%} & \accval{43.64\%} & \accval{24.52\%}
& \accval{46.87\%}\\
& \bc\textbf{LSVD-noQ}
& \bc\accval{\textbf{64.31\%}} & \bc\accval{\textbf{63.79\%}} & \bc\accval{\textbf{62.96\%}} & \bc\accval{\textbf{61.56\%}} & \bc\accval{\textbf{61.09\%}}
& \bc\accval{\textbf{62.74\%}}\\
\cline{3-8}
\rule{0pt}{2.75ex}
& \textcolor{gray}{FP16}
& \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 64.47\%}}
& \textcolor{gray}{64.47\%}\\

\midrule

\multirow{5.75}{*}{\rotatebox{90}{\makecell{Qwen2-VL\\7B}}}
& SVD-LLM
& \accval{79.12\%} & \accval{78.29\%} & \accval{73.92\%} & \accval{50.23\%} & \accval{20.83\%}
& \accval{60.48\%}\\
& QSVD-noQ
& \accval{80.16\%} & \accval{79.79\%} & \accval{76.69\%} & \accval{70.06\%} & \accval{64.51\%}
& \accval{74.24\%}\\
& WSVD-noQ
& \accval{80.68\%} & \accval{80.00\%} & \accval{76.31\%} & \accval{67.27\%} & \accval{52.81\%}
& \accval{71.41\%}\\
& \bc\textbf{LSVD-noQ}
& \bc\accval{\textbf{80.68\%}} & \bc\accval{\textbf{80.10\%}} & \bc\accval{\textbf{79.12\%}} & \bc\accval{\textbf{75.43\%}} & \bc\accval{\textbf{66.44\%}}
& \bc\accval{\textbf{76.35\%}}\\
\cline{3-8}
\rule{0pt}{2.75ex}
& \textcolor{gray}{FP16}
& \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 80.52\%}}
& \textcolor{gray}{80.52\%}\\

\midrule

\multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-v1.5\\7B}}}
& SVD-LLM
& \accval{55.22\%} & \accval{52.52\%} & \accval{47.01\%} & \accval{40.88\%} & \accval{31.06\%}
& \accval{45.34\%}\\
& QSVD-noQ
& \accval{61.25\%} & \accval{60.21\%} & \accval{60.17\%} & \accval{58.60\%} & \accval{56.56\%}
& \accval{59.36\%}\\
& WSVD-noQ
& \accval{60.82\%} & \accval{60.51\%} & \accval{59.94\%} & \accval{58.64\%} & \accval{56.61\%}
& \accval{59.30\%}\\
& \bc\textbf{LSVD-noQ}
& \bc\accval{\textbf{61.51\%}} & \bc\accval{\textbf{61.45\%}} & \bc\accval{\textbf{60.88\%}} & \bc\accval{\textbf{60.00\%}} & \bc\accval{\textbf{57.87\%}}
& \bc\accval{\textbf{60.34\%}}\\
\cline{3-8}
\rule{0pt}{2.75ex}
& \textcolor{gray}{FP16}
& \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 61.56\%}}
& \textcolor{gray}{\accval{61.56\%}}\\

\midrule

\multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-Next\\7B}}}
& SVD-LLM
& \accval{62.18\%} & \accval{61.04\%} & \accval{58.34\%} & \accval{55.95\%} & \accval{49.82\%}
& \accval{57.47\%}\\
& QSVD-noQ
& \accval{64.83\%} & \accval{64.36\%} & \accval{63.64\%} & \accval{62.08\%} & \accval{59.79\%}
& \accval{62.94\%}\\
& WSVD-noQ
& \accval{64.84\%} & \accval{64.83\%} & \accval{64.04\%} & \accval{64.10\%} & \accval{63.21\%}
& \accval{64.20\%}\\
& \bc\textbf{LSVD-noQ}
& \bc\accval{\textbf{64.99\%}} & \bc\accval{\textbf{65.09\%}} & \bc\accval{\textbf{64.88\%}} & \bc\accval{\textbf{64.94\%}} & \bc\accval{\textbf{64.26\%}}
& \bc\accval{\textbf{64.83\%}}\\
\cline{3-8}
\rule{0pt}{2.75ex}
& \textcolor{gray}{FP16}
& \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 65.14\%}}
& \textcolor{gray}{\accval{65.14\%}}\\

\midrule

\multirow{5.75}{*}{\rotatebox{90}{\makecell{LLaVA-Next\\13B}}}
& SVD-LLM
& \accval{65.09\%} & \accval{64.52\%} & \accval{61.40\%} & \accval{52.78\%} & \accval{44.05\%}
& \accval{57.57\%}\\
& QSVD-noQ
& \accval{67.27\%} & \accval{66.91\%} & \accval{66.86\%} & \accval{66.18\%} & \accval{63.95\%}
& \accval{66.23\%}\\
& WSVD-noQ
& \accval{67.48\%} & \accval{66.98\%} & \accval{66.86\%} & \accval{66.08\%} & \accval{65.14\%}
& \accval{66.51\%}\\
& \bc\textbf{LSVD-noQ}
& \bc\accval{\textbf{67.58\%}} & \bc\accval{\textbf{67.38\%}} & \bc\accval{\textbf{67.12\%}} & \bc\accval{\textbf{66.91\%}} & \bc\accval{\textbf{66.44\%}}
& \bc\accval{\textbf{67.09\%}}\\
\cline{3-8}
\rule{0pt}{2.75ex}
& \textcolor{gray}{FP16}
& \multicolumn{5}{c|}{\textcolor{gray}{Accuracy: 67.53\%}}
& \textcolor{gray}{\accval{67.53\%}}\\

\bottomrule
\end{tabular}%
}
\label{tab:mmb-en-fp16}
%\vspace{-8pt}
\end{table}
The MMBench EN V1.1 results in Tab.~\ref{tab:mmb-en-fp16} show the same trend on a different evaluation
benchmark. LSVD-noQ achieves the best average accuracy among low-rank methods
for all evaluated models. This indicates that the gains of LSVD are not limited
to ScienceQA-IMG or SEED-Bench, but also transfer to a more general multimodal
reasoning benchmark. In particular, LSVD-noQ remains close to the FP16 baseline
under mild compression and degrades more gracefully than prior SVD-based
methods under stronger compression.

\subsubsection{More Results in Quantized Settings}
\label{sec:appx-results-quant}
The low-precision results in Tab.~\ref{tab:appx-svd-result-quant} demonstrate that LSVD remains effective when
low-rank compression is combined with quantization. LSVD achieves the
highest average accuracy among all compressed low-precision methods, improving
over both quantization-only and SVD-based baselines. Compared with WSVD, LSVD
uses a more loss-aware decomposition, which better
preserves accuracy after quantization. The remaining gap to FP16 is small,
suggesting that LSVD provides a favorable trade-off between compression,
low-precision execution, and accuracy.

\begin{table}[h]
%\vspace{-12pt}
\centering
\small
\caption{Accuracy evaluation of different methods under low-precision on LLaVA-v1.5 and LLaVA-Next models.}
\label{tab:appx-svd-result-quant}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|c}
\toprule
\multirow{2}{*}{Method}
& \multicolumn{3}{c|}{ScienceQA-IMG $\uparrow$}
& \multicolumn{3}{c|}{SEED-Bench-IMG $\uparrow$}
& \multicolumn{3}{c|}{MMBench EN V1.1 $\uparrow$}
& \multirow{2}{*}{Avg. $\uparrow$} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
& v1.5 7B & Next 7B & Next 13B
& v1.5 7B & Next 7B & Next 13B
& v1.5 7B & Next 7B & Next 13B
& \\
\midrule
DuQuant
& 57.36\% & 66.34\% & 70.20\%
& 54.11\% & 63.64\% & 66.15\%
& 55.91\% & \textbf{62.78\%} & 64.31\%
& 62.31\% \\

QVLM
& 55.24\% & 60.60\% & 65.28\%
& 50.13\% & 50.38\% & 65.39\%
& 57.15\% & 60.29\% & 63.06\%
& 58.61\% \\

QSVD
& 65.61\% & 66.10\% & 70.43\%
& 58.49\% & 65.63\% & 69.21\%
& 45.45\% & 50.96\% & 45.56\%
& 59.72\% \\

WSVD
& 64.25\% & 66.94\% & \textbf{73.08\%}
& 60.23\% & 67.49\% & 70.67\%
& 56.57\% & 60.56\% & 64.68\%
& 64.94\% \\

\rowcolor{blue!10}
\textbf{LSVD}
& \textbf{66.14\%} & \textbf{68.37\%} & 72.11\%
& \textbf{61.94\%} & \textbf{67.49\%} & \textbf{71.56\%}
& \textbf{58.66\%} & 61.61\% & \textbf{65.08\%}
& \textbf{65.88\%} \\

\midrule
\textcolor{gray}{FP16}
& \textcolor{gray}{68.10\%} & \textcolor{gray}{69.60\%} & \textcolor{gray}{73.23\%}
& \textcolor{gray}{60.18\%} & \textcolor{gray}{69.02\%} & \textcolor{gray}{71.30\%}
& \textcolor{gray}{61.56\%} & \textcolor{gray}{65.14\%} & \textcolor{gray}{67.53\%}
& \textcolor{gray}{67.30\%} \\
\bottomrule
\end{tabular}%
}
%\vspace{-12pt}
\end{table}


% \newpage
\subsubsection{More Results for Ablation Studies}
\label{sec:appx-results-ablation}

\paragraph{Effectiveness of Quantization-aware Whitening}


\begin{wraptable}{r}{0.48\textwidth}
\vspace{-20pt}
\centering
\small
\caption{Results of quantization-aware whitening ablation.}
%\vspace{-5pt}
\resizebox{\linewidth}{!}{ %
\begin{tabular}{c|c|c|c|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{ScienceQA-IMG $\uparrow$} & \multirow{2}{*}{Avg. $\uparrow$} \\
\cmidrule{2-4}
& v1.5 7B & Next 7B & Next 13B & \\
\midrule
\textcolor{gray}{FP16}
& \textcolor{gray}{\accval{68.10\%}} 
& \textcolor{gray}{\accval{69.60\%}} 
& \textcolor{gray}{\accval{73.23\%}} 
& \textcolor{gray}{\accval{70.31\%}} \\

W/o QAW
& \accval{65.70\%} 
& \accval{68.07\%} 
& \accval{71.79\%} 
& \accval{68.52\%} \\

LSVD
& \accval{\textbf{66.14\%}} 
& \accval{\textbf{68.34\%}} 
& \accval{\textbf{72.11\%}} 
& \accval{\textbf{68.86\%}} \\
\bottomrule
\end{tabular}
}
\label{tab:quantization-aware-whitening-ablation}
%\vspace{-20pt}
\end{wraptable}

We evaluate quantization-aware whitening under the same W8A8 setting and compression ratio. The \textit{W/o QAW} baseline removes this component while keeping the rest of LSVD unchanged. As shown in Tab.~\ref{tab:quantization-aware-whitening-ablation}, QAW consistently improves accuracy across all models, raising the average from $68.52\%$ to $68.86\%$. This indicates that aligning the SVD transformation with the subsequent quantized execution helps preserve accuracy under low-precision compression.


%We evaluate the effectiveness of quantization-aware whitening under the same W8A8 setting and compression ratio. The \textit{W/o QAW} baseline removes quantization-aware whitening while keeping the remaining LSVD pipeline unchanged. As shown in Tab.~\ref{tab:quantization-aware-whitening-ablation}, quantization-aware whitening consistently improves accuracy across all evaluated models, increasing the average accuracy from 69.07\% to 69.51\%. This indicates that aligning the SVD transformation with the subsequent quantized execution helps preserve accuracy under low-precision compression.

\paragraph{Effectiveness of SVD-aware Permutation}

\begin{wraptable}{r}{0.48\textwidth}
% \vspace{-5pt}
\centering
\small
\caption{Results of SVD-aware permutation ablation.}
%\vspace{-5pt}
\resizebox{\linewidth}{!}{ %
\begin{tabular}{c|c|c|c|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{ScienceQA-IMG $\uparrow$} & \multirow{2}{*}{Avg. $\uparrow$} \\
\cmidrule{2-4}
& v1.5 7B & Next 7B & Next 13B & \\
\midrule
\textcolor{gray}{FP16}
& \textcolor{gray}{\accval{68.10\%}} 
& \textcolor{gray}{\accval{69.60\%}} 
& \textcolor{gray}{\accval{73.23\%}} 
& \textcolor{gray}{\accval{70.31\%}} \\

W/o Perm.
& \accval{58.80\%} 
& \accval{50.37\%} 
& \accval{67.92\%} 
& \accval{59.03\%} \\

LSVD
& \accval{\textbf{66.14\%}} 
& \accval{\textbf{68.34\%}} 
& \accval{\textbf{72.11\%}} 
& \accval{\textbf{68.86\%}} \\
\bottomrule
\end{tabular}
}
\label{tab:svd-aware-permutation-ablation}
%\vspace{-5pt}
\end{wraptable}

We evaluate the effectiveness of the SVD-aware permutation in the FFN (Sec.~\ref{sec:mix-quant-svd}) under the same setting as above. The \textit{W/o Perm.} baseline uses the same FFN SVD ratio as LSVD but does not group SVD-friendly channels before factorization. As shown in Tab.~\ref{tab:svd-aware-permutation-ablation}, removing this permutation reduces the average accuracy from $68.86\%$ to $59.03\%$, with a particularly large drop on LLaVA-Next 7B from $68.34\%$ to $50.37\%$. This shows that SVD-aware permutation effectively groups FFN channels that are more suitable for low-rank factorization, thereby preserving accuracy under FFN compression.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

\input{checklist.tex}


\end{document}
